Probabilistic Guarantees for Practical LIA Loop Invariant Automation

Despite the crucial need for formal safety and security verification of programs, discovering loop invariants remains a significant challenge. Static analysis is a primary technique for inferring loop invariants but often relies on substantial assumptions about underlying theories. Data-driven methods supported by dynamic analysis and machine learning algorithms have shown impressive performance in inferring loop invariants for some challenging programs. However, state-of-the-art data-driven techniques do not offer theoretical guarantees for finding loop invariants. We present a novel technique that leverages the simulated annealing (SA) search algorithm combined with SMT solvers and computational geometry to provide probabilistic guarantees for inferring loop invariants using data-driven methods. Our approach enhances the SA search with real analysis to define the search space and employs parallelism to increase the probability of success. To ensure the convergence of our algorithm, we adapt e-nets, a key concept from computational geometry. Our tool, DLIA2, implements these algorithms and demonstrates competitive performance against state-of-the-art techniques. We also identify a subclass of programs, on which we outperform the current state-of-the-art tool GSpacer.

==> sections/CHC-StateSpace-LIA.tex <==
\section{The state space and $d$-$c$-LIA invariants}
\label{Sec:Standard CHC clause and Classification of Datapoints}


Let $n$ be the number of integer variables in our programs (for some $n \in \mathbb{N}$). Then, the state space
$\mathcal{D}_{state}(n)$ is given by $\mathbb{Z}^n \cap [-\text{INT}\_\text{MAX} - 1, \text{INT}\_\text{MAX}]^n$ where $\text{INT}\_\text{MAX}$ is the largest integer that can be stored in our system. 
There is a partition of the state space, called the nil-unrolled partition ($0$U-partition) that classifies states into one of four sets: ground positive states ($+_g$), ground negative states ($-_g$), unknown inductive states ($?^{\rightarrow}$), and unknown noninductive states ($?^{\times}$). For the standard CHC system, these sets are defined below\footnote{If $S$ is an LIA formula, then the set of states represented by $S$ is given by $\{ \vec{x} \in \mathcal{D}_{state}(n) \: | \: S(\vec{x}) \}$.}: 
\begin{align*}
    +_g &:= P \\
    -_g &:= \neg Q \\
    ?^{\rightarrow} &:= B \land \neg (P \lor \neg Q) \\
    ?^{\times} &:= \neg (P \lor \neg Q) \setminus B
\end{align*}
We can check that the $0$U-partition forms a partition of $\mathcal{D}_{state}(n)$ iff $+_g \cap -_g = \varnothing$.
We additionally define ground implication pair states $\rightarrow_g$ (called ICE pairs in \cite{garg2014ice, garg2016learning}) by: $$\rightarrow_g := \{ (\vec{x}, \vec{y}) \in \mathbb{Z}^{2n} \: : \: \vec{x} \in ?^{\rightarrow} \land T(\vec{x}, \vec{y}) \}$$

We now describe the conditions for the standard CHC clause to admit an invariant. For this, we define an alter partition of the state space, called the completely unrolled partition (CU-partition) which classifies states into one of 3 sets: eventually positive states ($T^*(+_g)$), eventually negative states ($T^*(-_g)$) and neutral states ($0_g$). To define these sets, we need to first define the set of all $k$-reachable positive states $T^k(+_g)$ and $k$-reachable negative states $T^k(-_g)$ for all $k \in \mathbb{Z}_{\ge 0}$:
\begin{align*}
    T^0(+_g) &:= +_g \\
    T^0(-_g) &:= -_g \\
    k \ge 1 \Rightarrow T^{k}(+_g) &:= \{ y \: : \: (\exists x \in T^{k-1}(+_g) \land B) \: T(x,y)  \} \\
    k \ge 1 \Rightarrow T^{k}(-_g) &:= \{ x \: : \: (x \in B) \land ((\exists y \in T^{k-1}(-_g) ) \: T(x,y))  \}
\end{align*}
Then we have:
\begin{align*}
     T^*(+_g) &:= \bigcup_{k \ge 0}  T^k(+_g) \\
     T^*(-_g) &:= \bigcup_{k \ge 0}  T^k(-_g) \\
     0_g &:= \neg (T^*(+_g) \cup T^*(-_g))
\end{align*}
We can check that the CU-partition forms a partition of $\mathcal{D}_{state}(n)$ iff $T^*(+_g) \cap T^*(-_g) = \varnothing$. An important distinction between the $0$U-partition and the CU-partition is that the partition sets of the $0$U-partition are always recursive whereas for the unbounded CHC clause system, $T^*(+_g)$ and $T^*(-_g)$ are recursively enumerable in general, and $0_g$ is co-recursively enumerable in general~\cite{blass2001inadequacy}.
For the code example in Fig~\ref{eg1}, we show the $0$U-partition and the CU-partition in Fig~\ref{Fig:$0$U and CU}. 
Lemma~\ref{Lemma: Admit Invariant} gives the exact criterion for the standard CHC system to admit an invariant, which we prove in Appendix~\ref{App: Standard CHC Clause and State Space Lemmas and Proofs.}.  

\begin{figure}
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/0U-partition.png}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/CU-partition.png}
\end{minipage}
\caption{The $0$U and CU-partition for the program example in Fig~\ref{eg1}. In the plot for the $0$U-partition (left), the green plus represents the sole ground positive state, the red minuses represent negative states, and the blue dots represent unknown inductive states (As $B = \top$ for this example, there are no unknown noninductive states). In the plot for the CU-partition (right), the green pluses represent the eventually positive states, the red minuses represents the eventually negative states, and the yellow dots represent the neutral states.  }
\label{Fig:$0$U and CU}
\end{figure}

\begin{lemma} \label{Lemma: Admit Invariant}
The standard CHC system admits a loop invariant iff $T^*(+_g) \cap T^*(-_g) = \varnothing$. 
\end{lemma}




By Lemma \ref{Lemma: Admit Invariant}, to prove a standard CHC system doesn't admit an invariant requires us to show the existence of a state $\vec{x} \in T^*(+_g) \cap T^*(-_g)$ - which usually requires dynamic trace collection and/or fuzzing, which is a different paradigm within program verification. Hence, we make an additional assumption that the standard CHC system should admit an invariant. As $T^*(+_g) \cap T^*(-_g) = \varnothing \Rightarrow +_g \cap -_g = \varnothing$, hence our assumption on the standard CHC clause implies that the $0$U-partition is indeed a partition of the state space. 
% \saeid{I feel that we need to say something different here: maybe we want to say the invariants in the CU-partition are
% sound (over-approximation of  $0$U-partition?), esp if we are going to work with CU-partition.} \ak{We work with 0U-partition, CU-partition is the ideal partition which we can never find, we need it to statme some lemmas which gives motivation like why we assume our program admits invariant, every invariant is $d$-$c$ LIA invariant etc.}

Using the CU-partition of the state space, we can alternatively define a loop invariant $I$ as a subset of the state space which contains $T^*(+_g)$, excludes $T^*(-_g)$, and is $T$-inductive on $0_g \cap B$, i.e., $\vec{x} \in 0_g \cap B \cap I) \land T(\vec{x}, \Vec{y}) \Rightarrow \vec{y} \in I$. 
% \saeid{could not follow the T-closed part: let's discuss in the next meeting.} \ak{ $T$-closed -> $T$-inductive } 
Lemma~\ref{Lemma: Lattice} states the complete lattice structure of all invariants that we prove in Appendix~\ref{App: Standard CHC Clause and State Space Lemmas and Proofs.}.

\begin{lemma} \label{Lemma: Lattice}
If $T^*(+_g) \cap T^*(-_g) = \varnothing$, the set of all loop invariants satisfying the standard CHC clause forms a complete lattice $\Lambda$ w.r.t implication.     
\end{lemma}

Lemma~\ref{Lemma: Lattice} implies that we can talk about a `strongest' invariant for the standard CHC system (which is the infimum of $\Lambda$). Let LIA invariant be a formula in LIA theory, which is also an invariant of the standard CHC system. Lemma~\ref{Lemma: I is LIA I } (see proof in Appendix~\ref{App: Standard CHC Clause and State Space Lemmas and Proofs.}) says that as our state space is comprised of a finite number of lattice points, any invariant is logically equivalent to some LIA invariant. 

\begin{lemma} \label{Lemma: I is LIA I }
If $\mathcal{D}_{state}(n) = \mathbb{Z}^n \cap [-\text{INT}\_\text{MAX} - 1, \text{INT}\_\text{MAX}]^n$, then every invariant $I$ of the standard CHC clause is logically equivalent to some LIA invariant. Together with Lemma \ref{Lemma: Lattice}, this implies that if $T^*(+_g) \cap T^*(-_g) = \varnothing$, the set of all LIA invariants forms a complete lattice w.r.t implication.
\end{lemma}

In addition to assuming that our standard CHC system admits an LIA invariants (follows from Lemma \ref{Lemma: I is LIA I }), 
% \saeid{one or more such invariants?} \ak{we assume it admits atleast one invariant.}
we consider fixed-size LIA invariants, specifically $d$-$c$ LIA invariants:

\begin{definition} \label{Def: dc LIA I}
Given $d,c \in \mathbb{N}$, a $d$-$c$ LIA invariant  is a formula of the form 
$$ \bigvee_{i=1}^d \bigwedge_{j=1}^c \vec{w}_{ij}^T \vec{x} \le b_{ij}~~~~where~~~~~~ \vec{w}_{ij} \in \mathbb{Z}^n ~and~b_{ij} \in \mathbb{Z}~for~all~i~and~j.$$
\end{definition}

It is important to note that we only allow the `$\le$' operator in a $d$-$c$ LIA invariant. 
\saeid{does the next sentence explain why?} \ak{Lemma 4.5 explains why - it explains why only restricting to $\le$ operator is good enough.} \saeid{maybe we should move this to the end of paragraph?}
Geometrically, a $d$-$c$ LIA invariant is an invariant that is the union of the lattice points contained in $d$ compact polytopes in $\mathbb{R}^n$, where each polytope has at most $c$ faces. Finally, Lemma~\ref{Lemma: LIA is dcLIA} states that as our state space has only lattice points, any LIA invariant is logically equivalent to a $d$-$c$ LIA invariant for some $d,c \in \mathbb{N}$ (see proof in Appendix \ref{App: Standard CHC Clause and State Space Lemmas and Proofs.}).
% \saeid{what does logically equivalent mean?} \ak{standard bi-implication operator $P \leftrightarrow Q$}

\begin{lemma} \label{Lemma: LIA is dcLIA}
If $\mathcal{D}_{state}(n) \subseteq \mathbb{Z}^n$, then every LIA invariant of the standard CHC clause system is logically equivalent to a $d$-$c$ LIA invariant for some $d,c \in \mathbb{N}$.    
\end{lemma}

The $d$ and $c$ of the LIA invariant are called the `disjunctive size' and the `conjunctive size' of the $d$-$c$ LIA invariant respectively. While we use decision trees to support users to judiciously pick appropriate values for $d$ and $c$ (see Section \ref{Sec:Tool and Experiments}); we generally assume that these values are set by the user. 

\begin{definition}[{\bf Problem Statement}] \label{Def: problem}
\saeid{here, we need to include a problem statement that precisely states what are the given and what problem we try to solve in the next section, etc. Can we state the problem s.t. doing SA and DS look natural solution to the problem without mentioning them?}
\end{definition}


==> sections/Convergence.tex <==
\section{Convergence Guarantees}
\label{Sec:Convergence Guarantees}


We first show that the DS Loop can run foratmost a bounded number of iterations with some minimum probability in Theorem \ref{DS Loop bound} which we prove in Appendix \ref{Proofs in Convergece Guarantees}. For this, we define the dimension of a set $S \subseteq \mathbb{Z}^n$.

\begin{definition}
    Let $S \subseteq \mathbb{Z}^n$. Then the dimension of $S$ is the dimension of the smallest flat in $\mathbb{R}^n$ containing $S$.
\end{definition}

\begin{theorem} \label{DS Loop bound}
    Let $n \in \mathbb{N}$ be the number of integer variables in the program. If $P = \cup_{i=1}^{d_P} \mathcal{P}_i^+$ , $\neg Q = \cup_{i=1}^{2^{c_Q}} \mathcal{P}_i^-$ and $B  = \cup_{i=1}^{d_B} \mathcal{P}_i^{?_\rightarrow}$ where $\mathcal{P}_i^+$, $\mathcal{P}_i^-$ and $\mathcal{P}_i^{\rightarrow}$ are compact polytopes in $\mathbb{Z}^n$ for all i, then let us assume that the dimension of $\mathcal{P}_i^+$, $\mathcal{P}_i^-$ and $\mathcal{P}_i^{\rightarrow}$ is either $n$ or $0$ forall $i$. Then with probability atleast $\delta^{d_0}$, the DS Loop terminates within $s_{\text{ep}} \cdot \lceil \log_2 (\epsilon_0 n^n \# \mathcal{P}^*) \lceil + d_0 \cdot (n!V_0 + n) + 1$ where $d_0 := \max (d_P, d_B, 2^{c_Q})$ and $\# \mathcal{P}^* := \max (\max_i \# \mathcal{P}^+_i, \max_i \# \mathcal{P}^{\rightarrow}_i, \max_i \# \mathcal{P}^-_i)$ and $\# S$ denotes the number of lattice points contained in set $S$. 
\end{theorem}
We note that the $n \log_2 n$ sum can be dropped from the above bound to get an upper bound of $s_{\text{ep}} \cdot \log_2 (\epsilon_0) +  s_{\text{ep}} \cdot \log_2 (\# \mathcal{P}^*)$ by using the ranges as polytopes\footnote{An upper bound to the number of faces of the polytope can be computed using Lemma \ref{Lemma: CEX spaces}, which is required to bound the VC dimension of the polytopes} instead of ellipsoids. However, in practice this slows each iteration of the SA run as $\epsilon$-nets w.r.t polytopes (of the required number of faces) is much larger than an $\epsilon$-net w.r.t ellipsoids. Note that our method allows us to get a much faster bound than $O(\log_2 \# \mathcal{P}^*)$ by the following simple observation: Let $h: \mathbb{N} \rightarrow \mathbb{N}$ be any function, and let the scheme to constrict an epsilon net be given by $\epsilon_k = \frac{\epsilon_0}{h(k)}$. For such a scheme, our bound on the number of DS iterations is given by  $O(h^{(-1)} ( \# \mathcal{P}^* ))$. Hence for any choice of $h$ which grows faster than the exponential function, say a double exponential function or Ackermann function, we get a faster bound on the number of DS iterations. Additionally note that if we set $\epsilon_0 < \frac{1}{\mathcal{P}^*}$, we converge by the first DS iteration - however an $\epsilon_0$ so small also increases the iteration time of the SA run. As a balance we use the the exponential function as our choice of $h$ and set $\epsilon_0 = \frac{1}{2}$.

We next show that any run of the SA Loop in any iteration of the DS Loop finds an approximate invariant with some minimum probability in Theorem \ref{SA loop prob}. 

\begin{theorem} \label{SA loop prob}
    Let $n \in \mathbb{N}$ be the number of integer variables and let $t_{max}$ be the number of iterations for which SA runs. Then if $t_{max} \ge ??$, SA converges to an invariant with probability atleast $p_0 = ?? $. Moreover, if $|TS|$ is the size of the training set for this SA run, then the worst case time for a full SA search in atmost $t_{max}$ steps is $ ??$.
\end{theorem}

Combining the above two results, we get the full guarantees for our tool:
\begin{theorem}
    \toolname{} finds an invariant in atmost $\chi = s_{\text{ep}} \cdot \lceil \log_2 (\epsilon_0 n^n \# \mathcal{P}^*) \lceil + d_0 \cdot (n!V_0 + n) + 1$ Z3 calls and the total probability of success is given by $p_0^{\chi}$ where $p_0 = ??$. Moreover, this computation takes $ ?? $ time.
\end{theorem}

==> sections/Experiments.tex <==
\section{Tool and Experiments}\label{Sec:Tool and Experiments}
\subsection{Implementation.}
We have implemented \toolname in Python. We manually convert verification benchmarks into CHC clauses and feed in the CHC clause as the input. We manually pick tasks from SV-COMP 2023~\cite{svbenchmark} that can be represented as CHCs with LIA and have an LIA loop invariant. The evaluation results are shown in \autoref{table:benchmark}.


\begin{table}[!h]
\begin{center}
\caption{\label{table:benchmark}Numbers of SA iterations and Z3 calls for each benchmark solved by \toolname (best out of 3 rounds). Time-out is indicated by "-".}

% -------------------------------------------------------------
% |||||||||||||||||||||||||||||||||||||||||||||||||||||||||||||
% The following content is generated by src/extract-table.ipynb
% |||||||||||||||||||||||||||||||||||||||||||||||||||||||||||||
% -------------------------------------------------------------
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Benchmark & SA & DS & Benchmark & SA & DS \\
\hline
handcrafted/c2d1\_1 & 4176 & 3 & loop\_zilu/benchmark21\_disjunctive & 647 & 2 \\
handcrafted/mock & 287 & 4 & loop\_zilu/benchmark22\_conjunctive & - & - \\
loop\_lit/afnp2014\_modified & 1652 & 8 & loop\_zilu/benchmark23\_conjunctive & - & - \\
loop\_lit/bhmr2007 & - & - & loop\_zilu/benchmark24\_conjunctive & 83725 & 10 \\
loop\_lit/cggmp2005 & - & - & loop\_zilu/benchmark25\_linear & 167 & 4 \\
loop\_lit/cggmp2005\_variant & - & - & loop\_zilu/benchmark26\_linear & 225 & 1 \\
loop\_lit/gsv2008 & 393 & 2 & loop\_zilu/benchmark27\_linear & 1413 & 5 \\
loop\_lit/gj2007 & - & - & loop\_zilu/benchmark28\_linear & 732 & 3 \\
loop\_lit/gj2007b & - & - & loop\_zilu/benchmark29\_linear & 3404 & 13 \\
loop\_lit/hhk2008 & - & - & loop\_zilu/benchmark30\_conjunctive & 3157 & 7 \\
loop\_lit/jm2006 & - & - & loop\_zilu/benchmark31\_disjunctive & 1831 & 5 \\
loop\_lit/jm2006\_variant & - & - & loop\_zilu/benchmark32\_linear & 103 & 1 \\
loop\_new/count\_by\_1 & - & - & loop\_zilu/benchmark33\_linear & 9 & 1 \\
loop\_new/count\_by\_1\_variant & - & - & loop\_zilu/benchmark34\_conjunctive & - & - \\
loop\_simple/nested\_1 & 124 & 2 & loop\_zilu/benchmark35\_linear & 23 & 1 \\
loop\_zilu/benchmark01\_conjunctive & 493 & 2 & loop\_zilu/benchmark36\_conjunctive & 8 & 1 \\
loop\_zilu/benchmark02\_linear & 590 & 2 & loop\_zilu/benchmark37\_conjunctive & 206 & 1 \\
loop\_zilu/benchmark03\_linear & - & - & loop\_zilu/benchmark38\_conjunctive & 124617 & 6 \\
loop\_zilu/benchmark04\_conjunctive & 9600 & 11 & loop\_zilu/benchmark39\_conjunctive & 8468 & 7 \\
loop\_zilu/benchmark05\_conjunctive & 13452 & 7 & loop\_zilu/benchmark40\_polynomial & 4722 & 3 \\
loop\_zilu/benchmark06\_conjunctive & - & - & loop\_zilu/benchmark41\_conjunctive & - & - \\
loop\_zilu/benchmark07\_linear & - & - & loop\_zilu/benchmark42\_conjunctive & 152797 & 8 \\
loop\_zilu/benchmark08\_conjunctive & 6526 & 9 & loop\_zilu/benchmark43\_conjunctive & 145153 & 10 \\
loop\_zilu/benchmark09\_conjunctive & 21 & 1 & loop\_zilu/benchmark44\_disjunctive & - & - \\
loop\_zilu/benchmark10\_conjunctive & 1029 & 4 & loop\_zilu/benchmark45\_disjunctive & 1393 & 3 \\
loop\_zilu/benchmark11\_linear & 251 & 1 & loop\_zilu/benchmark46\_disjunctive & 14091 & 3 \\
loop\_zilu/benchmark12\_linear & 157 & 1 & loop\_zilu/benchmark47\_linear & 484 & 3 \\
loop\_zilu/benchmark13\_conjunctive & 14250 & 3 & loop\_zilu/benchmark48\_linear & 580 & 3 \\
loop\_zilu/benchmark14\_linear & 110 & 1 & loop\_zilu/benchmark49\_linear & 1374 & 5 \\
loop\_zilu/benchmark15\_conjunctive & 276512 & 5 & loop\_zilu/benchmark50\_linear & 305 & 1 \\
loop\_zilu/benchmark16\_conjunctive & 31182 & 6 & loop\_zilu/benchmark51\_polynomial & 5829 & 2 \\
loop\_zilu/benchmark17\_conjunctive & 1547 & 5 & loop\_zilu/benchmark52\_polynomial & 2188 & 3 \\
loop\_zilu/benchmark18\_conjunctive & 84293 & 9 & loop\_zilu/benchmark53\_polynomial & 4650 & 5 \\
loop\_zilu/benchmark19\_conjunctive & - & - & loops\_crafted\_1/Mono1\_1\_2 & - & - \\
loop\_zilu/benchmark20\_conjunctive & 82899 & 5 & loops\_crafted\_1/Mono3\_1 & - & - \\
\hline
\end{tabular}
}
% ---------------------------------------------------------
% |||||||||||||||||||||||||||||||||||||||||||||||||||||||||
% The above content is generated by src/extract-table.ipynb
% |||||||||||||||||||||||||||||||||||||||||||||||||||||||||
% ---------------------------------------------------------

\end{center}
\end{table}

\subsection{Hyperparameter Fitting.}
We give the value of hyperparameters we choose for our research below: 
\begin{itemize}
    \item Number of Variables ($n$): This is inferred from the program input. In the case when we learn affine spaces, we don't reduce the number of variables $n$
    \item Maximum Modulus Coefficient Coordinate (k):We set $k$ according to Lemma \ref{Lemma: Connected Rot Graph}.
    \item Maximum Rotation Angle ($\theta_0$): We set $\theta_0 = \frac{\pi}{4}$ as the minimum angle so that $G_{\mathcal{R}}(n,k, \theta_0)$ is connected forall $n$ and $k$.
    \item Maximum translation distance ($t_0$): We set $t_0 = 10$.
    \item Conjunctive and Disjunctive Size (c, d): We note that we could pick any value greater than or equal to the minimum conjunctive and disjunctive size required, and such an invariant will exist, although the candidate search space will grow larger. \textcolor{red}{We fill the following ML formula}
    \item Maximum single threaded SA steps ($t_{max}$): We set $t_{max} = 10^7$ according to our computations on Lemma 
    \item Number of threads ($p$): We set $p = 4$.
    \item Checking Window size ($t_{window}$): We set $t_{window} = 1000$ as a fine balance between running the other threads for too long after some thread has found the approximate invariant, and checking at each time step for each thread which becomes too time expensive.
    \item Number of cex per clause ($s$): We set $s = 5$.
    \item Verifier: Z3
    
\end{itemize}
\subsection{Benchmarking.}



\subsection{Comparison with Dynamic Algorithms.}
We compare \toolname with LinearArbitrary, to get the following:

\textbf{Any 3: LinearArbitrary, Code2Inv, LoopInvgen, ICE-DT: 'Learning Invariants using Decision Trees
and Implication Counterexamples', ''}

\begin{itemize}
\item \textbf{Size of Invariant.} Invariant found by LinearArbitray may be way too large. For a program, they found:
\begin{figure}
\includegraphics[scale=0.25]{sections/8.png}
\end{figure}
wheras we found:
\begin{figure}
\includegraphics[scale=.75]{sections/81.png}
\end{figure}
Neither invariants are stronger than one another. \\
\item Unsound results for real input.
\item Don't use ICE pairs. Hence the following example can only be solved by their algorithm in a hit and trial fashion. Start with $P$ as a triangle and let it move along straight path, so that after a large number of iterations, there is a change in the transition function, then they shouldn't be able to guess final invariant because they will have no information about this change.
\end{itemize}

\subsection{Comparison with Static Algorithms.}

\textbf{ Spacer , Duality, UAtomizer }

Static Algorithms like Abstract Interpretation only work for a limited class of linear invariants. For example Daikon only finds conjunctive invariants (no disjunctions allowed) using atomic predicates which occur in the program. As such static algorithms come with better completeness and computation time guarantees, but only for the class of invariants for which they work on.

\subsection{Comparison with Randomized Algorithms.}
The only randomized algorithm tool is C2I. The comparison is as follows: 
\begin{itemize}
\item They use Metropolis Hashing on the invariant space where the neighbourhood function can change the actual set by a huge difference - this ensures that any cost function designed on this space will have a huge number of local minimas, and any search based algorithm will have poor results.\footnote{ They actually uniformly pick a predicate out of a fixed formula with $c = d = 10$ and randomly change a coefficient of constant value to ANY possible value allowed by their domain with probability $1 -p$ and with probablity $p$ remove the predicate altogether.}
\item Their cost function does not give smooth feedback\footnote{A serious limitation is that it is positive semidefinite instead of positive definite; also had to correct their formula for ICE pairs.} They have:
\begin{align*}
c(I) &= \sum_{+} \neg I(+) + \sum_{+} \neg I(-) + \sum_{(h,t)} \neg \neg I(+) * I(-) + \\ &\sum_+ \sum_-  I(+) \cdot I(-) + \neg I(+) \cdot \neg I(-)
\end{align*}
\item No $\epsilon$-nets implies no guarantee for convergence of CEGIS loop except by a finiteness argument.
\item Only ran on 8 programs, and they report convergence in 0.0 seconds for 5 of them indicating that their starting point is very close to the actual invariant.
\end{itemize}
\subsection{Analysis of Performance.} \label{Subsec: Analysis of Performance}

There are two main reasons for non-convergence. First, in some cases, the number of Z3 runs may be too large. This specially happens in the case of $n = 1$, and we have to do a large linear search over a ray.

The other case is when we are required to search for affine spaces in a SA search. As any equality is represented as two inequalities in a LIA invariant, it is harder to find invariants which contain an affine predicate.

The third is coarse-grained rotations. We try to make our rotations more fine grained.

THe fourth is the centre of rotation: the foot of perpendicular from the origin won't lie on the face for polytopes located further from origin, or shaped at extreme vertex angles. In such a case, we do a rotation about a farther away point, and hence the set size changes by quite a bit.

==> sections/Method.tex <==
\section{Methodology}
\label{Sec:Algorithm}
Our algorithm to find a $d$-$c$ LIA invariant involves a Simulated Annealing (SA) Loop nested inside a Datapoint Sampling (DS) Loop.
The DS Loop samples datapoints from the standard CHC clause to find an approximate CHC system. The SA Loop finds an approximate invariant to this approximate CHC system. The DS Loop then checks if the approximate invariant is a true invariant of the standard CHC system. If it is, then the DS Loop halts, else the DS Loop updates the datapoints sampled to get a `better' approximate CHC system. This process continues till we find a invariant of the SA Loop or the SA Loop returns `Fail'.

We describe the DS loop and SA loop individually in subsection \ref{SubSec:CEGIS Loop} and \ref{SubSec:SA Loop} respectively. We give the pseudocode of the full algorithm in Algorithm \ref{Alg: Full}. Note that the preprocessing for the algorithm includes two steps - (1) computing the hyperparameters and (2) Computing a computation-heavy graph called the `rotation graph' which is used and is described in the SA-Loop.

\begin{algorithm}[H]
\caption{Full Algorithm}
\label{Alg: Full}
\begin{algorithmic}[1]
\State \textbf{Input: } $(P, B, T, Q)$
\State Compute Hyperparameters
\State Compute the Rotation Graph $G_{\mathcal{R}}$
\State Return DS\_Loop (P, B, T, Q)
\end{algorithmic}
\end{algorithm}




\subsection{Datapoint Sampling Loop}\label{SubSec:CEGIS Loop}
\saeid{We need to take one step back and say what is the high-level goal and how we will achieve them. For example, the goal is to verify a candidate invariant satisfies the CHC system...}
The goal of the DS loop is to compute plus points $+ \subseteq +_g$, minus points $- \subseteq -_g$ and implication pairs $\rightarrow \subseteq \rightarrow_g$ s.t. a $d$-$c$ LIA invariant $I$ to the $(+, -, \rightarrow)$-approximate CHC system defined by: 
 \begin{align*} \label{App CHC}
(\forall \vec{s} \in  +) \: P(\vec{s}) &\rightarrow I(\vec{s}) \\
(\forall (\vec{s},\vec{s'}) \in \: \rightarrow) \:  I(\vec{s}) \land B(\vec{s}) \land T(\vec{s},\vec{s'}) &\rightarrow I(\vec{s'})  \\
(\forall \vec{s} \in -) \: I(\vec{s})  &\rightarrow Q(\vec{s})  
\end{align*}
is a `good' approximation to some $d$-$c$ LIA invariant $I_0$ of the standard CHC system; where a `good' approximation is interpreted as the value $|I \: \Delta \: I_0|$ being `small' ($\Delta$ is the set symmetric difference operator). Such an invariant $I$ is called a $(+, -, \rightarrow)$-approximate $d$-$c$ LIA invariant. \saeid{this paragraph is not clear, particularly what is $I_0$, good, small, etc.}

For the $(k + 1)^{\text{th}}$ $(k \in \mathbb{Z}_{\ge 0})$ iteration of the DS loop, we compute a set of plus points $(+_k)$, minus points $(-_k)$ and implication pairs $(\rightarrow_k)$, collectively known as the training set $(S_k := (+_k, -_k, \rightarrow_k))$, which we input to the SA loop. For this section, we treat the SA loop as a blackbox which takes as input the $S_k$-approximate CHC system, and outputs either a $S_k$-approximate $d$-$c$ LIA invariant $I'$ or `Fail'. If the SA loop outputs `Fail', we halt the DS loop reporting `Fail'. If the SA loop outputs a $S_k$-approximate invariant $I'$, we check if $I'$ satisfies the standard CHC clause using an SMT solver.  As our formulas are in LIA theory (where satisfiability and validity is decidable), an SMT solver can check if $I'$ is an invariant or not. If $I'$ is an invariant to the standard CHC system, then we halt the DS loop and report $I'$ as our found invariant. But if $I'$ is not an invariant of the standard CHC system, we compute $S_{k+1} = (+_{k+1}, -_{k+1}, \rightarrow_{k+1}))$ and move on to the next iteration of the DS Loop. We give a pseudocode of the DS Loop in Algorithm~\ref{alg: DS Loop}.
\saeid{this is a bit confusing because it sounds like we are putting two procedures together.}

\begin{algorithm}[H]
\caption{DS Loop}\label{alg: DS Loop}
\begin{algorithmic}[1]
\State \textbf{Input: } $(P, B, T, Q)$
\State Compute $S_0 = (+_0, -_0, \rightarrow_0)$
\While {$\top$} 
\State $k \leftarrow 0$
\State (SUCCESS, I) $\leftarrow$ SA\_LOOP( $S_k$-approximate CHC clause, $k$)
\If{SUCCESS = `Fail'}
\State Return `Fail'
\EndIf
\State (VERIFY, Z3) $\leftarrow$ SMT\_VERIFER( I, Standard CHC clause)
\If{VERIFY = `True'}
\State Return I
\EndIf
\State Compute $S_k = (+_k, -_k, \rightarrow_k)$
\State $k \leftarrow k + 1$
\EndWhile
\end{algorithmic}
\end{algorithm}

\subsubsection{Initial Training Set.}
In order to define $S_0 = (+_0, -_0, \rightarrow_0)$,
\saeid{It sounds like the initial set can be a separate subsection entirely, so we have three parts: initial, SA, and Z3.}


 We now define a compact polytope in $\mathbb{Z}^n$.
\begin{definition}
     A compact polytope in $\mathbb{Z}^n$ is defined as the set of all lattice points contained in a compact polytope $S$ in $\mathbb{R}^n$. Furthermore, $S$ is referred to as the associated real polytope of the compact polytope in $\mathbb{Z}^n$.
\end{definition}

By the Minkowski-Weyl theorem, any vector in a compact polytope in $\mathbb{R}^n$ can be written as the convex combination of it's vertices\footnote{A vertex of a compact polytope $\mathcal{P}$ is a point which does not lie in any open line segment contained in $\mathcal{P}$.}. However as the vertices of a compact polytope in $\mathbb{R}^n$ need not be lattice points, some of these vertices need not lie in our state space. This motivates us to define lattice vertices of a compact polytope in $\mathbb{Z}^n$.

\begin{definition}
    Let $\mathcal{P}$ be a compact polytope in $\mathbb{Z}^n$ and let $\mathcal{P}'$ be it's associated real polytope. If $E_\mathbb{Z}$ denotes the set of all vertices of $\mathcal{P}'$ which are lattice points, and $E_\mathbb{R}$ denotes the set of all vertices of $\mathcal{P}'$ which are not lattice points, then the lattice vertices of $\mathcal{P}$, denoted by $E_{\Lambda}(\mathcal{P})$, are defined by:
    $$E_{\Lambda}(\mathcal{P}) = E_\mathbb{Z} \cup \bigcup_{\vec{v} \in E_\mathbb{R}} \{ \vec{u} \in \mathcal{P} \: : \: || \vec{u} - \vec{v} ||_{\infty} \le 1\} $$
where $ || \cdot ||_{\infty}$ refers to the $L\infty$ norm on $\mathbb{R}^n$.
\end{definition}
To find the lattice vertices of a compact polytope $\mathcal{P}$ in $\mathbb{Z}^n$, we use an ILP solver to find all vertices of it's associated real polytope. Furthermore, for every non-lattice point vertices $v$, we check all lattice points contained within a unit $L_{\infty}$ ball centered at $v$ for membership in $\mathcal{P}$. Finally, we define a CEX-net of a compact polytope in $\mathbb{Z}^n$ w.r.t a set of ranges $\mathcal{R}$.

\begin{definition}
    For any compact polytope $\mathcal{P}$ in $\mathbb{Z}^n$, $0 < \epsilon < 1$,  $0 < \delta < 1$, $V_0 > 0$, and a set of ranges $\mathcal{R}$ with bounded VC dimension, a CEX-net for $\mathcal{P}$ w.r.t $\mathcal{R}$ for hyperparameters $\delta, \epsilon, V_0$, denoted CEX-net$(\mathcal{P}; V_0, \epsilon, \delta, \mathcal{R})$, is a randomized $\epsilon$-net of $\mathcal{P}$ w.r.t $\mathcal{R}$ with probability atleast $\delta$, if the n dimensional volume of $\mathcal{P}$ is greater than $V_0$; and the set of lattice vertices of $\mathcal{P}$, if the n dimensional volume of $\mathcal{P}$ is atmost $V_0$. 
\end{definition}

A CEX-net for a compact polytope $\mathcal{P}$ w.r.t $\mathcal{R}$ is a more `practical' approximation of $\mathcal{P}$ than a $\epsilon$-net of $\mathcal{P}$ w.r.t $\mathcal{R}$ for the following reason: The size of a randomized $\epsilon$-net for $\mathcal{P}$ w.r.t $\mathcal{R}$ with probability at least $\delta$ is independent of the size of $\mathcal{P}$, and is quite large. If $\mathcal{P}$ has only a few points to start with (this condition can be roughly checked for full dimensional polytopes $\mathcal{P}$ by comparing the n-dimensional volume of $\mathcal{P}$ to some threshold $V_0$), then an $\epsilon$-net for $\mathcal{P}$ w.r.t $\mathcal{R}$ may almost be equal to $\mathcal{P}$ itself - in this case, the lattice vertices for $\mathcal{P}$ suffice as a good `approximation' of $\mathcal{P}$. Additionally, if $\mathcal{P}$ is contained in some affine space of dimension less than $n$, then computing a randomized $\epsilon$-net for $\mathcal{P}$ w.r.t $\mathcal{R}$ via rejection sampling is inefficient as the sampling time is too high (see Appendix \ref{App: Rejection Sampling}). In this case, too, we must take the lattice vertices for $\mathcal{P}$ as an `approximation' of $\mathcal{P}$ (note that when $\mathcal{P}$ is not full dimensional, it's $n$ dimensional volume is $0$).

Now we can define our sets $+_0$, $-_0$ and $\rightarrow_0$.
First note that by our assumption that $P$, $B$ and $Q$ are LIA formulas, we have $P$, $\neg Q$ and $B$ to be the finite union of compact polytopes in $\mathbb{Z}^n$ i.e let $P = \cup_i \mathcal{P}_i^+$, $\neg Q = \cup_i \mathcal{P}_i^-$ and $B = \cup_i \mathcal{P}_i^{\rightarrow}$ where $\mathcal{P}_i^+$, $\mathcal{P}_i^-$ and $\mathcal{P}_i^{\rightarrow}$ are compact polytopes in $\mathbb{Z}^n$ for all i. Let $\mathcal{E}$ be a class of sets where each $e \in \mathcal{E}$ is the set of lattice points in some $n$ dimensional ellipsoid in $\mathbb{R}^n$. 

Then we define:
\begin{align*}
    +_0 &:= \bigcup_{i} \text{CEX-net$(\mathcal{P}_i^+; V_0, \epsilon_0, \delta, \mathcal{E})$} \\
    -_0 &:= \bigcup_{i} \text{CEX-net$(\mathcal{P}_i^-; V_0, \epsilon_0, \delta, \mathcal{E})$} \\
    \rightarrow_0 &:= \bigcup_{i} \{ (x,y) \: | \: x \in \text{CEX-net$(\mathcal{P}_i^{\rightarrow}; V_0, \epsilon_0, \delta, \mathcal{E})$} \land T(x,y) \}   
\end{align*}
for some choice of hyperparameters $V_0$, $\epsilon_0$ and $\delta$.
To motivate our choice of ranges to be the lattice points contained in some $n$-dimensional ellipsoid, we first describe the counterexample-space of each clause in the standard CHC clause w.r.t a $(+, -, \rightarrow)$-approximate invariant in Lemma \ref{Lemma: CEX spaces} (see Appendix \ref{App: Proofs for Lemmas in Methodology} for proof).  

\begin{lemma} \label{Lemma: CEX spaces}
    Let $+ \subseteq +_g$, $- \subseteq -_g$ and $\rightarrow \: \subseteq \: \rightarrow_g$ s.t. $I$ is a $(+, -, \rightarrow)$ approximate invariant. Then, we have:
\begin{itemize}
    \item The set of counterexamples to the fact clause $(C1)$ of the standard CHC system w.r.t $I$ is given by the set of ground positive points $P \land \neg I \subseteq +_g$. 
    \item The set of counterexamples to the inductive clause $(C2)$ of the standard CHC system w.r.t $I$ is given by the set of ground implication pairs $\{ (x,y) \: : \: (x \in I \land B \land T^{-1}(\neg I) ) \land T(x,y) \} \subseteq \: \rightarrow_g$ where $T^{-1}(S) := \{ x \: : \: (\exists y \in S) \: T(x,y) \}$. \saeid{can you double check this one if this gives counterexample?} \ak{was a typo; fixed it.}
    \item The set of counterexamples to the query clause $(C3)$ of the standard CHC system w.r.t $I$ is given by the set of ground negative states $I \land \neg Q \subseteq -_g$. 
\end{itemize}
Additionally, if $P$, $B$ and $Q$ are LIA formulas, $T$ is a piecewise linear relation over $B$ with integer coefficients and $I$ is a $d$-$c$ LIA invariant, then $P \land \neg I$, $I \land B \land T^{-1}(I)$ and $I \land \neg Q$ are the finite union of compact polytopes in $\mathbb{Z}^n$. \saeid{should not be $P \land \neg I$?} \ak{\checkmark}
\end{lemma}

As each counterexample space to $(C1)$, $(C2)$ and $(C3)$ w.r.t. any $(+, -, \rightarrow)$-approximate invariant is a finite union of compact polytopes in $\mathbb{Z}^n$, ideally, we would want to take our ranges of the CEX-nets used in the definition of $+_0$, $-_0$ and $\rightarrow_0$ to be compact polytopes in $\mathbb{Z}^n$ as such a choice would ensure that the size of any compact polytope in $\mathbb{Z}^n$ in a counterexample space of $(C1)$, $(C2)$ or $(C3)$ is bounded above, as we ensure $+_0 \subseteq +$, $-_0 \subseteq -$ and $\rightarrow_0 \: \subseteq \rightarrow$. But as the counterexample spaces themselves are the finite union of compact polytopes in $\mathbb{Z}^n$, this would ensure that the sizes of the counterexample spaces $(C1)$, $(C2)$ and $(C3)$ are itself bounded above. However as the VC dimension of a compact polytope in $\mathbb{Z}^n$ with at most $c$ faces is less than or equal to $2c(n+1) \log(3c)$ \cite{blumer1989learnability}, which is quite large, we get that the size of a CEX-net for a polytope w.r.t compact polytopes in $\mathbb{Z}^n$ as ranges to be very large, which leads to a very slow search speed in the SA loop. As a workaround, we note that every compact polytope in $\mathbb{R}^n$ has a unique inscribed and circumscribing $n$-dimensional ellipsoid called the inner and outer Lowner-John Ellipsoids, and the VC dimension of class of $n$-dimensional ellipsoids in $\mathbb{R}^n$ is $\frac{n^2 + 3n}{2}$ \cite{akama2011vc}, which is much lower than the VC dimension of compact polytopes in $\mathbb{Z}^n$ for small $n$ values. Hence, if we take our ranges to be the lattice points contained in any $n$-dimensional ellipsoid\footnote{The VC dimension of the class of lattice points contained in an $n$-dimensional ellipsoid is trivially less than the VC dimension of the class of $n$-dimensional ellipsoids in $\mathbb{R}^n$.}, we ensure that the number of lattice points in any inner Lowner-John Ellipsoid of any compact polytope in the counterexample space to $(C1)$, $(C2)$ and $(C3)$ w.r.t $I$ is bounded above. This further implies that the size of any compact polytope in the counterexample space is bounded above (albeit a weaker bound than the one provided by using compact polytope in $\mathbb{Z}^n$ as ranges), and as before, this upper bounds the size of our entire counterexample space. We finally end this discussion by defining the relation between the inner and outer Lowner-John ellipsoids of a polytope and the polytope in Definition \ref{Def JL Ellipsoids}. 

\begin{lemma}\cite{henk2012lowner} \label{Def JL Ellipsoids}
    Let $\mathcal{P}$ be a compact polytope. Then there exists an ellipsoid $E$ centred at origin, a vector $\vec{t}$ called the centre s.t. the inner and outer Lowner-John ellipsoids of $\mathcal{P}$ are given by $\vec{t} + \frac{1}{n}E$ and $\vec{t} + E$ respectively \saeid{potential typo!} \ak{fixed}, where $\frac{1}{n}E$ is the n-dimensional ellipsoid $E$ dilated by a factor of $\frac{1}{n}$. Then we have:
    $$\vec{t} + \frac{1}{n}E \subseteq \mathcal{P} \subseteq \vec{t} + E $$
\end{lemma}
\saeid{we should say a bit more explicitly how everything together helps us come up with the initial points.}

\subsubsection{Subsequent Training Sets.}
Let $S_k := (+_k, -_k, \rightarrow_k)$ denote the training set computed at the $(k+1)^{\text{th}}$ iteration of the DS loop. Suppose the SA Loop finds a $S_{k-1}$ approximate $d$-$c$ LIA invariant $I'$ which is not an invariant of the standard CHC clause. Then we use two strategies to compute $S_{k}$, namely Learning Counterexamples and Constricting CEX-nets.
\begin{itemize}
    \item \textit{Learning Counterexamples.}  Forall iterations $k$, we additionally query the SMT solver for $s \in \mathbb{N}$ distinct counterexamples to $(C1)$, $(C2)$, and $(C3)$. Sampling a distinct counterexample to the CHC clause $(Ci)$ w.r.t $I'$ for any $i \in \{ 1,2,3 \}$, after already having sampled $T^{\times}$ distinct counterexamples for $(Ci)$ can be done by asking the SMT solver to produce a satisfiable state to the following equation:
$$ \bigwedge_{t \in T^{\times}} ( x \neq t) \land \neg (Ci)(I_k) $$
In the formula above, $x$ is a state for the $(C1)$ and $(C3)$ clauses, and a pair of states for the $(C2)$ clause. Let $+_k^{\times}$ ,$-_k^{\times}$ and $\rightarrow_k^{\times}$ denote the the counterexamples generated to $(C1)$, $(C2)$ and $(C3)$ w.r.t $I'$ at the $(k+1)^{\text{th}}$ iteration of the DS loop respectively.
\item \textit{Constricting CEX-nets.} We periodically decrease the $\epsilon$ of the CEX-net computed at the start of the DS Loop. Let $P = \cup_i \mathcal{P}_i^+$, $\neg Q = \cup_i \mathcal{P}_i^-$ and $B = \cup_i \mathcal{P}_i^{\rightarrow}$ where $\mathcal{P}_i^+$, $\mathcal{P}_i^-$ and $\mathcal{P}_i^{\rightarrow}$ are compact polytopes in $\mathbb{Z}^n$ for all i. Then for some hyperparameter $s_{\text{ep}}$ called the epoch size, forall $k \in \mathbb{Z}_{\ge 0}$, at iteration $ks_{\text{ep}} + 1$, we compute the sets, $(+_{ks_{\text{ep}}}^{\epsilon}, -_{ks_{\text{ep}}}^{\epsilon}, \rightarrow_{ks_{\text{ep}}}^{\epsilon})$ defined below.
\begin{align*}
    +_{ks_{\text{ep}}}^{\epsilon} &:= \bigcup_{i} \text{CEX-net$(\mathcal{P}_i^+; V_0, \frac{\epsilon_0}{2^k}, \delta, \mathcal{E})$} \\
    -_{ks_{\text{ep}}}^{\epsilon} &:= \bigcup_{i} \text{CEX-net$(\mathcal{P}_i^-; V_0, \frac{\epsilon_0}{2^k}, \delta, \mathcal{E})$} \\
    \rightarrow_{ks_{\text{ep}}}^{\epsilon} &:= \bigcup_{i} \{ (x,y) \: | \: x \in \text{CEX-net$(\mathcal{P}_i^{\rightarrow}; V_0, \frac{\epsilon_0}{2^k}, \delta, \mathcal{E})$} \land T(x,y) \}   
\end{align*}
where $\mathcal{E}$ is the class of sets of lattice points in some $n$ dimensional ellipsoid. Note that given a CEX-net with parameters $V_0, \epsilon, \delta, \mathcal{E}$ for some compact polytope in $\mathbb{Z}^n$, you can find a CEX-net with parameters $V_0, \frac{\epsilon}{2}, \delta, \mathcal{E}$ by at-most adding a few randomly sampled points to the previous CEX-net. Hence, we can always ensure forall $k$, 
 $+_{(k-1)s_{\text{ep}}}^{\epsilon} \subseteq +_{ks_{\text{ep}}}^{\epsilon}$, $-_{(k-1)s_{\text{ep}}}^{\epsilon} \subseteq -_{ks_{\text{ep}}}^{\epsilon}$ and $\rightarrow_{(k-1)s_{\text{ep}}}^{\epsilon} \subseteq \rightarrow_{ks_{\text{ep}}}^{\epsilon}$.
\end{itemize} 

Then for the $k + 1$th iteration, we compute the training set $S_{k}$ at the beginning of this iteration, by the following scheme:
 \begin{align*}
      +_{k} &:=  \begin{cases}
          +_{k-1} \cup +^\times_{k-1} \cup +_{k}^{\epsilon} &\text{$k$ is a multiple of $s_{\text{ep}}$} \\
          +_{k-1} \cup +^\times_{k-1} &\text{o.w.} \\
      \end{cases} \\
      -_{k} &:=  \begin{cases}
          -_{k-1} \cup -^\times_{k-1} \cup -_{k}^{\epsilon} &\text{$k$ is a multiple of $s_{\text{ep}}$} \\
          -_{k-1} \cup -^\times_{k-1} &\text{o.w.} \\
      \end{cases} \\
      \rightarrow_{k} &:=  \begin{cases}
          \rightarrow_{k-1} \cup \rightarrow^\times_{k-1} \cup \rightarrow_{k}^{\epsilon} &\text{$k$ is a multiple of $s_{\text{ep}}$} \\
          \rightarrow_{k-1} \cup \rightarrow^\times_{k-1} &\text{o.w.} 
      \end{cases} 
 \end{align*}
 Once we compute $S_{k}$, we proceed to the next iteration of the DS loop. Note that this strategy ensures $(\forall k)$ $+_k \subseteq +_{k+1}$, $-_k \subseteq -_{k+1}$, and $\rightarrow_k \: \subseteq \: \rightarrow_{k+1}$ which implies that $(\forall k)$ $(\exists \epsilon)$ $+_{k'}^{\epsilon} \subseteq +_k$, $-_{k'}^{\epsilon} \subseteq -_k$, and $\rightarrow_{k'}^{\epsilon} \: \subseteq \: \rightarrow_k$ where $k' := \lceil \frac{k}{s} \rceil$. Hence forall $k$, the plus, minus and implication pairs of $S_k$ contains an $\epsilon$ net for each polytope of $P$ , $\neg Q$ and $B$ respectivly, for some $\epsilon \in (0,1)$.

\subsection{Simulated Annealing Loop}\label{SubSec:SA Loop}

The goal of our SA loop is to find a $(+,-,\rightarrow)$ approximate invariant given a $(+, - , \rightarrow)$ approximate CHC clause. Prior to defining our algorithm for multi-threaded SA search, we first introduce a standard (single-threaded) simulated annealing search to define some terminologies. 

A standard (single-threaded) simulated annealing search takes a finite search space $\mathcal{S}$, a symmetric neighbor relation $\mathcal{N}$ on $\mathcal{S}$, a non-negative cost function $V: \mathcal{S} \rightarrow [0, \infty)$, and a starting point $s_0 \in \mathcal{S}$ as inputs; and aims to find a global minimum $s^*$ of $V$ by the following Algorithm~\ref{alg:Standard Single Thread SA Search}. 

\begin{algorithm}[!tbh]
\caption{Standard Single Thread SA Search}
\begin{algorithmic}[1]
\State \textbf{Input: } $(\mathcal{S}, \mathcal{N}, V, s_0)$
\State \textbf{HyperParameters: } ($t_{max}$, $T_0$)
\State Set $s \leftarrow s_0$ and compute $V \leftarrow V(s_0)$
\While {$0 \le j \le t_{max}$} 
\State Uniformly sample a neighbor $s'$ of $s$ from $\mathcal{N}(s)$.
\State Let temperature $T_j \leftarrow \frac{T_0}{\ln (1 + j)}$
\State Compute $V' \leftarrow V(s')$
\State With probability $p = \frac{1}{|\mathcal{N}(I)|} \cdot e^{-\frac{(V' - V)^+}{T_j}}$  set $s \leftarrow s'$ and $V \leftarrow V'$
\If {$V = 0$} 
\State Return $I$
\EndIf
\EndWhile
\State Return `Fail'
\end{algorithmic}
\label{alg:Standard Single Thread SA Search}
\end{algorithm}

Now we define the search space, the neighborhood relation, the cost function, and the starting point for our SA loop.

\subsubsection{Candidate Invariant Space and Neighbourhood Relation}
Our SA search space is called the candidate invariant space, and any element of this space is called a candidate invariant. To define the candidate invariant space, we first define the rotation graph $G_{\mathcal{R}}(n ;k, \theta_0) = (V_{\mathcal{R}}(n; k), E_{\mathcal{R}}(n;k, \theta_0))$ for some $k \in \mathbb{N}$ and $\theta_0 \in (0, \pi]$ by:
\begin{align*}
    V_{\mathcal{R}}(n ; k) &:= \{ (u_1, u_2, ... u_n) \: | \: (\forall i \: u_i \in \mathbb{Z}_{[-k,k]}) \land (u_1, u_2, ... u_n) \neq \vec{0} \land \gcd (|u_1|, |u_2|, ... |u_n|) = 1 \} \\
    E_{\mathcal{R}}(n ;k, \theta_0) &:= \{ (\vec{u}, \vec{v})  \: | \:  \vec{u}, \vec{v} \in V_{\mathcal{R}}(n;k) \land 0 < \arccos  \frac{\vec{u} \cdot \vec{v}}{||\vec{u}|| ||\vec{v}||}   \le \theta_0 \}
\end{align*}
$k$ and $\theta_0$ are called the maximum absolute coefficient value and maximum rotation angle respectively. 

It is trivial to see that $ \frac{(2k+1)^n - 1}{k} \le |V_{\mathcal{R}}(n;k)| < (2k+1)^n$. Computing $G_{\mathcal{R}}(n;k, \theta_0)$ takes $O(|V_{\mathcal{R}}|^2) = O((2k+1)^{2n})$ time, which is why we precompute the rotation graphs for a few frequently used $n$, $k$ and $\theta_0$ values and simply load this graph in the pre-processing stage of the algorithm. \saeid{Is this first time that we talk about this? If yes, I can rephrase this.} \ak{Yes, first time talking about this.} We note that the large computation time of the rotation graph only allows us to set smaller values of $k$, which we discuss in Section \ref{Subsec: Analysis of Performance} to be the major factor that negatively affects the experimental performance of our method. \saeid{let us remove the last sentence after `to be major...' and talk about it in the experimental section.
Rather, let us talk about the positive aspect of it: how did we manage to precompute the graphs for any search?} \ak{we compute it using naive brute force; i.e. computing the edges of any graph with v vertices takes $O(v^2)$ time.}

We next show any vertex of $G_{\mathcal{R}}(n,k, \theta_0)$ has bounded degree in Lemma \ref{Lemma: rotation degree bound} which we prove in Appendix $\ref{App: Proofs for Lemmas in Methodology}$. 

\begin{lemma} \label{Lemma: rotation degree bound}
 Let $\theta_0 \in (0, \frac{\pi}{2})$ and $\vec{u} \in V_{\mathcal{R}}(n;k)$. If $d_{\mathcal{R}}(\vec{u})$ denote the number of neighbors of $\vec{u}$ in $G_{\mathcal{R}}(n;k, \theta_0)$, then 
$$d_{\mathcal{R}}(\vec{u}) \le \frac{1}{n} \cdot  \Bigg( 2k \cdot \Big\lceil\frac{ \sin \theta_0}{\cos \theta_0 \cos (\theta_0 + \gamma_z) } \Big\rceil+ \frac{3}{2} \Bigg)^{n}$$ 
where $\gamma = \arccos \frac{\min_i |u_i|}{||\vec{u}||^2}$.
\end{lemma}





We next show that $G_{\mathcal{R}}(n;k, \theta_0)$ is connected for a large enough value of $\theta_0$ in Lemma \ref{Lemma: Connected Rot Graph} which we prove in Appendix $\ref{App: Proofs for Lemmas in Methodology}$. 


\begin{lemma} \label{Lemma: Connected Rot Graph}
    Forall $n$ and $k$, if $\theta_0 \ge \arccos \frac{k}{\sqrt{k^2 + \max (1 , \frac{n-1}{4}) }}$,  then $G_{\mathcal{R}}(n ; k, \theta_0)$ is connected forall $n$ and $k$.
\end{lemma}

Given $c, d, k_1 \in \mathbb{N}$, we define our candidate invariant space $\mathcal{S}(n; c, d, k, k_1)$, as the set of all $d$-$c$ LIA formulas with coefficient vectors from $V_{\mathcal{R}}(n;k)$ and integer constants from $[-k_1, k_1]$ i.e.
\begin{align*}
\mathcal{S}(n; c, d, k, k_1) &:= \Big\{ \bigvee_{i = 1}^d \bigwedge_{j=1}^c (\vec{w}_{ij} \cdot \vec{x} \le b_{ij})  \: : \: (\forall i j) \: \vec{w}_{ij} \in V_{\mathcal{R}}(n,k) \land b_{ij} \in \mathbb{Z}_{[-k_1, k_1]} \Big\},    
\end{align*}
where $d$ and $c$ are called the disjunctive and conjunctive sizes of the candidate invariant space, respectively; and $k_1$ is called the maximum absolute constant value. We note that each candidate invariant $I := \bigvee_{i = 1}^d \bigwedge_{j=1}^c (\vec{w}_{ij} \cdot \vec{x} \le b_{ij})$ corresponds to a set of points in $\mathcal{D}_{state}(n)$ given by $\{ \vec{s} \in \mathcal{D}_{state}(n) \: : \:  \bigvee_{i = 1}^d \bigwedge_{j=1}^c (\vec{w}_{ij} \cdot \vec{s} \le b_{ij}) \}$


Next we define the (symmetric) neighbourhood relation on $\mathcal{S}(n; c, d, k, k_1)$ denoted by $\mathcal{N}(n ;c,d, k, k_1, t, \theta_0)$ for some $t \in \mathbb{N}$, which is called the maximum translation distance, as:

Given $I, I' \in \mathcal{S}(n; c, d, k, k_1)$, $(I,I') \in \mathcal{N}(n; c,d, k, k_1, t, \theta_0)$ iff $\exists i_0 \in [1,d] \: \exists j_0 \in [1,c]$ s.t. if $I =  \bigvee_{i = 1}^d \bigwedge_{j=1}^c (\vec{v}_{ij} \cdot \vec{x} \le a_{ij})$ and $I' =  \bigvee_{i = 1}^d \bigwedge_{j=1}^c (\vec{w}_{ij} \cdot \vec{x} \le b_{ij})$, then we must both of the following conditions to hold:
\begin{enumerate}
    \item All but one atomic predicate is different i.e. $(\forall i ) \: (\forall j) ((i,j) \neq (i_0, j_0)) \Rightarrow (\vec{v_{ij}} = \vec{w_{ij}} ) \land (a_{ij} = b_{ij})$ AND,
    \item The different atomic predicates are either rotations or translations of each other i.e.
    \begin{itemize}
        \item Atomic Predicates are translations of each other: $\vec{v}_{i_0j_0} = \vec{w}_{i_0j_0}$ and $0 < |a_{i_0j_0} - b_{i_0j_0} | \le t||\vec{v}_{i_0j_0}||$ OR,
        \item Atomic Predicates are rotations of each other:
        $(\vec{v}_{i_0j_0} , \vec{w}_{i_0j_0}) \in E_{\mathcal{R}}(n;k,\theta_0)$ and $b_{i_0j_0} = \big\lfloor a_{i_0j_0} \frac{\vec{v_{i_0j_0}} \cdot \vec{w_{i_0j_0}}}{||\vec{v_{i_0j_0}}||^2} \big\rfloor $ or $b_{i_0j_0} \in \Big[ \big\lceil a_{i_0j_0} \frac{||\vec{w_{i_0j_0}}||^2}{\vec{v_{i_0j_0}} \cdot \vec{w_{i_0j_0}}}\big\rceil, \big\lceil (a_{i_0j_0} + 1) \cdot \frac{||\vec{w_{i_0j_0}}||^2}{\vec{v_{i_0j_0}} \cdot \vec{w_{i_0j_0}}}\big\rceil \Big]$. We motivate this choice of constant of rotation. Consider a rotation scheme where we set $b_{i_0j_0} =  a_{i_0j_0} \frac{\vec{v_{i_0j_0}} \cdot \vec{w_{i_0j_0}}}{||\vec{v_{i_0j_0}}||^2} $. This is a rotation of $(\vec{v}_{i_0j_0} \cdot \vec{x} \le a_{i_0j_0})$ to $(\vec{w}_{i_0j_0} \cdot \vec{x} \le b_{i_0j_0})$ where the center of rotation is the foot of the perpendicular from the origin to $(\vec{v}_{i_0j_0} \cdot \vec{x} \le a_{i_0j_0})$. But as we need $b_{i_0j_0} \in \mathbb{Z}$, we must alter the rotaion scheme to take $b_{i_0j_0} = \big\lceil a_{i_0j_0} \frac{\vec{v_{i_0j_0}} \cdot \vec{w_{i_0j_0}}}{||\vec{v_{i_0j_0}}||^2} \big\rceil$. But now, this rotation scheme need not be symmetric, hence we take the symmetric closure of this rotation scheme and allow transitions to $(\vec{w}_{i_0j_0} \cdot \vec{x} \le c)$ for all integer constants $c$ where a rotation from $(\vec{w}_{i_0j_0} \cdot \vec{x} \le c)$ to $(\vec{v}_{i_0j_0} \cdot \vec{x} \le a_{i_0j_0})$ is allowed by the before mentioned rotation scheme - these constants $c$ are precisely the integers in the closed interval $\Big[ \big\lceil a_{i_0j_0} \frac{||\vec{w_{i_0j_0}}||^2}{\vec{v_{i_0j_0}} \cdot \vec{w_{i_0j_0}}}\big\rceil, \big\lceil (a_{i_0j_0} + 1) \cdot \frac{||\vec{w_{i_0j_0}}||^2}{\vec{v_{i_0j_0}} \cdot \vec{w_{i_0j_0}}}\big\rceil \Big]$.
    \end{itemize}
\end{enumerate}



\subsubsection{Cost Function}

Given $I\in \mathcal{S}(n; c, d, k, k_1)$, and a training set $S = (+, -, \rightarrow)$, 
we define the cost of $I$ denoted by $V( I ; +, -, \rightarrow )$ as:

$$V( I ; +, -, \rightarrow ) :=   \ \sum_{\vec{p} \in +} \delta(I, \vec{p}) + \sum_{\vec{n} \in -} \delta(\neg I, \vec{n}) + \sum_{(\vec{hd},\vec{tl}) \in \rightarrow} \min( \delta(\neg I, \vec{hd}), \delta (I, \vec{tl}) ) $$ 
where if $E := \bigvee_{j=1}^d \bigwedge_{i=1}^c \vec{w_{ij}}^T x \le b_{ij}$, 
% \saeid{should not be $\neg I$ for pos?} \ak{No, when $p \in I$, cost should be 0.}
then
$$(\forall \vec{s}) \: \delta ( E , \vec{s} ) := \min_{1 \le j \le d} \sum_{i=1}^c \frac{(\vec{w_{ij}}^T \vec{s} - b_{ij})^+}{||\vec{w_{ij}}||} $$ 
where $(x)^+ := \max (x ,0)$. Also note that if $I := \bigvee_{j=1}^d \bigwedge_{i=1}^c \vec{w_{ij}}^T x \le b_{ij}$, then $\neg I = \bigvee_{j=1}^{2^c} \bigwedge_{i=1}^d - \vec{w}_{i\sigma_j(i)}^T x \le - b_{i\sigma_j(i)} - 1$ where $\{ \sigma_{j} \}_{j=1}^{2^c}$ is the set of all $2^c$ permutations on $[1,c]$, hence $\delta ( \neg I , \vec{s} )$ is well defined forall $\vec{s}$.

Intuitively if $I\in \mathcal{S}(n; c, d, k, k_1)$ for any $c, d \in \mathbb{N}$, $\delta (I; \vec{s} )$ is an approximation to the Euclidean distance of $\vec{s}$ from the set of points in $\mathcal{D}_{state}(n)$ corresponding to $I$. Hence, $V(I; +, -, \rightarrow)$ measures the fitness of $(+, -, \rightarrow)$ in approximating the invariant $I$. We note that 
Lemma \ref{Lemma: Properties of delta}, which we prove in Appendix \ref{App: Proofs for Lemmas in Methodology},
shows the non-negativity of $\delta$, zero values when the property $\vec{s} \in I$ holds true,
the over-approximation of actual Euclidean distance by a factor of $c$, and the linear-time computable properties of
$\delta ( I , \vec{s} )$.

\begin{lemma} \label{Lemma: Properties of delta}
$(\forall \vec{s} \in \mathcal{D}_{state}(n))$ $(\forall c, d, k, k_1)$ $(\forall I \in \mathcal{S}(n; c, d, k, k_1))$, $\delta(I,\vec{s})$ satisfies the following properties:
\begin{enumerate}
\item Non-negativity:  $\delta(I,\vec{s}) \ge 0 $.
\item Zero only for $\vec{s} \in I$:  $\vec{s} \in I \Leftrightarrow \delta(I,\vec{s}) = 0$.
\item $c$-over approximation to actual Euclidean distance from $\vec{s}$ to $I$: If $d_I(\vec{s}) = \inf \{ || \vec{s} -  \vec{t}|| \: : \:  \vec{t} \in I \} $ represents the actual Euclidean distance of $\vec{s}$ from $I$, then we have $\frac{\delta(I,\vec{s})}{d_I(\vec{s})} \le c $ 
\item Linearly computable: $\delta(I,\vec{s})$ can be computed in $O(ncd)$ time.
\end{enumerate}    
\end{lemma}

Lemma \ref{Lemma: Properties of delta} implies the non-negativity, zeroness iff $I$ is a $(+,-,\rightarrow)$-approximate invariant, and computing speed of $V( I ; +, -, \rightarrow )$, which we note in Lemma \ref{Lemma: Properties of V} and prove in Appendix \ref{App: Proofs for Lemmas in Methodology}.

\begin{lemma} \label{Lemma: Properties of V}
    $(\forall c, d, k, k_1)$, $(\forall I \in \mathcal{S}(n; c, d, k, k_1))$, $\forall (+, -, \rightarrow)$, $V(I; +, -, \rightarrow)$ satisfies the following properties:
\begin{enumerate}
    \item Non negativity: $V(I; +, -, \rightarrow) \ge 0$
    \item Zero iff $I$ is a $(+, -, \rightarrow)$-approximate invariant. 
    \item Computing $V(I; +, -, \rightarrow)$ takes $O(n2^cd \cdot |S|)$ where $|S| := |+| \: + \: |-| \: + \: |\rightarrow|$. 
\end{enumerate}
\end{lemma}

\subsubsection{Starting Point}
We now describe the starting point for the SA loop. We make a different choice for the starting point of the SA loop depending on the iteration count $k$ of the DS loop, which we denote by $I_0(k)$. 
\begin{itemize}
    \item $k = 0$: We compute $I_0(0)$ by uniformly sampling each coefficient of each atomic predicate $I_0(0)$ from $V_{\mathcal{R}}(n,k)$ and setting each constant to $0$ i.e.
$$ I_0(0) \leftarrow \bigvee_{j=1}^d \bigwedge_{i=1}^c w_{ij}^Tx \le 0 \: : (\forall i j) \: w_{ij} \sim U(V_{\mathcal{R}}(n,k)) $$
where $U(S)$ represents a uniform distribution over the set $S$.
We base this choice of starting candidate invariant according to the small constants principle used in \cite{pldi/2016/PadhiSM}: \textit{Candidate invariants with small absolute constant values are more likely to be approximate invariants.} \saeid{I find this a bit hard to imagine. why is there $V$? should not we use something about eps-net here?}
    \item $k > 0$: We set $I_0(k)$ to the $S_{k-1}$-approximate invariant output by the SA loop in the $(k-1)^{\text{th}}$ iteration of the DS loop. This ensures that the search for the loop invariant in the $k^{\text{th}}$ SA Loop starts from where the $(k-1)^{\text{th}}$ SA Loop ends.
\end{itemize}


\subsubsection{Multi-threaded SA Search on Nested Candidate Invariant Spaces.} We now give the multi-threaded simulated search algorithm. We use $p \in \mathbb{N}$ independent threads in the SA loop, where $p$ is a hyper-parameter. For each $i$ in $1 \le i \le p$, we have a parameter $k_1(i) \in \mathbb{N}$ such that the $i^{\text{th}}$ thread runs on a candidate invariant space whose maximum absolute constant value is $k_1(i)$, which is denoted by $\mathcal{S}_i(n; c, d, k, k_1(i))$. Note that if for any two threads $i$ and $j$, $k_1(i) < k_1(j)$, then the candidate invariant space for the $i$th thread is contained in the candidate invariant space for the $j$th thread i.e. $$k_1(i) < k_1(j) \Rightarrow \mathcal{S}_i(n; c, d, k, k_1(i)) \subset \mathcal{S}_j(n; c, d, k, k_1(j))$$
This ensures a higher probability of finding approximate invariants with small absolute constant values - a heuristic motivated by the small constants principle mentioned before. Additionally, we note in Lemma \ref{Lemma: Max abs const value} (proof in Appendix \ref{App: Proofs for Lemmas in Methodology}) that $\mathcal{S}(n; c, d, k, k_1)$ is large enough to represent any $d$-$c$ LIA invariant if $k_1 = nk(INT\_MAX + 1)$. For this, we first define the notion of logical equivalence of two formulas under a set $S$ in Definition \ref{Def: Logical Equivalence under S}.

\begin{definition} \label{Def: Logical Equivalence under S}
    Let $S$ be any set. Let $F_1$ and $F_2$ be quantifier-free first-order formulas over the free variables $s$ which take values in $S$. Then $F_1$ and $F_2$ are logically equivalent under $S$, denoted $F_1 \leftrightarrow_S F_2$ if $\{ \vec{s} \in S \: : \: F_1(s)\} = \{ \vec{s} \in S \: : \: F_2(s)\}$.
\end{definition}


\begin{lemma} \label{Lemma: Max abs const value}
  $\forall (n, c, d, k$), if $I$ is a $d$-$c$ LIA invariant, then: 
  $$ (\exists I' \in \mathcal{S}(n; c, d, k,  nk(INT\_MAX + 1))) \: I \leftrightarrow_{\mathcal{D}_{\text{state}(n)}} I'$$ .  
\end{lemma}

We always ensure one thread runs on the candidate invariant space with the maximum absolute constant value equal to $nk(INT\_MAX + 1)$. For the remaining threads $1 \le i \le p - 1$, we pick some parameters $1 \le k_1(1) < ... \: k_1(p-1) < nk(INT\_MAX + 1)$ as the maximum absolute constant values of their respective candidate invariant spaces.
Note that each thread does a SA search in it's own candidate invariant space, with the same state space and data-points, the same cost function as defined above and with it's own starting point chosen with the scheme mentioned before.

We now describe the algorithm for the SA loop which uses $p$ threads. We use two thread-shared lists of length $p$ called $rv\_list$ and $I\_list$, where the $i$th entry of $rv\_list$ and $I\_list$ stores the return value and the starting point of the $i$th thread respectively. We initialize the $i$th entry of these lists to `None' and $I_0$ respectively. We create $p$ threads via the FORK procedure and make each thread run a modified version of the standard single threaded SA search  which we describe later. We then make the calling function to wait for the termination of all $p$ threads by the JOIN procedure, and finally check if any of the threads find an approximate invariant. If they do, we output that as the return value of our SA Loop, else we output `Fail'. We give the pseudo-code of the SA Loop in Algorithm \ref{SMultiA-Algorithm}.

\begin{algorithm}
\caption{SA Loop}\label{SMultiA-Algorithm}
\begin{algorithmic}[1]
\State \textbf{Input: } $(+, -, \rightarrow); (\forall j) \: I_0^{(j)}$
\State \textbf{Hyperparameters: } $p$
\State $(\forall 1 \le i \le p) \: rv\_list[i] \leftarrow `None'$
\State $(\forall 1 \le i \le p) \: I\_list[i] \leftarrow I_0^{(i)}$
\State $(\forall 1 \le i \le p) \: FORK( \text{Modified Single Threaded SA Search}(+, -, \rightarrow, I_0^{(i)}, rv\_list, I\_list, i))$
\State $(\forall 1 \le i \le p) \: JOIN( i)$
\If {$\exists k \: rv\_list[k] \neq `None'$}
\State Return $I\_list[k]$
\EndIf
\State Return `Fail'
\end{algorithmic}
\end{algorithm}

We now describe the modified version of the single threaded SA search which is used in the SA Loop algorithm. The algorithm is similar to the standard single threaded SA search, with the addition that once a thread finds an approximate invariant, it updates it's corresponding $rv\_list$ and $I\_list$ entry. All threads check these shared lists periodically at multiples of $t_{window}$ steps, and if any invariant has found an approximate invariant, they force halt. The pseudo-code of the modified single thread SA search is given in Algorithm \ref{Alg: Modified SA search}. It calls two functions, STORE and CHECK whose pseudocode are given in Algorithm \ref{Alg: STORE} and Algorithm \ref{Alg: CHECK} respectively. The STORE function stores the invariant and return value of thread $i$ into it's respective $I\_list$ and $rv\_list$ entry; and the CHECK function checks if any approximate invariant is stored in $rv\_list$ and if so, forcefully times out the thread running it, after storing it's current candidate invariant value to it's $I\_list$ entry.

\begin{algorithm}
\caption{Modified Single Thread SA Search} \label{Alg: Modified SA search}
\begin{algorithmic}[1]
\State \textbf{Input: } $(+, -, \rightarrow, I_0, rv\_list, I\_list, i)$
\State \textbf{HyperParameters: } ($t_{max}$, $T_0, t_{window}$)
\State Set $I \leftarrow I_0$ and compute $V \leftarrow V(I_0)$

\If {$V = 0$} 
STORE(I, I, $rv\_list$, $I\_list$, $i$), Return $I$
\EndIf

\While {$0 \le j \le t_{max}$} 
\State CHECK(j, $rv\_list$, $I\_list$, $i$)
\State Uniformly sample a neighbor $s'$ of $s$ from $\mathcal{N}(s)$.
\State Let temperature $T_j \leftarrow \frac{T_0}{\ln (1 + j)}$
\State Compute $V' \leftarrow V(I')$
\State With probability $p = \frac{1}{|\mathcal{N}(I)|} \cdot e^{-\frac{(V' - V)^+}{T_j}}$;  set $I \leftarrow I'$ and $V \leftarrow V'$
\If {$V = 0$} STORE(I, I, $rv\_list$, $I\_list$, $i$), Return $I$
\EndIf
\EndWhile
\State STORE($I_{t_{max}}$, `None', $rv\_list$, $I\_list$, $i$), Return `Fail'
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{CHECK Procedure} \label{Alg: CHECK}
\begin{algorithmic}[1]
\State \textbf{Input: } $j$, $rv\_list$, $I\_list$, $i$
\If {$j \% t_{window} = 0 \land (\exists k) \: rv\_list[k] \neq `None'$ }
\State $I\_list[i] \leftarrow I^{(i)}_j$
\State Return $I^{(i)}_j$
\EndIf
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{STORE procedure} \label{Alg: STORE}
\begin{algorithmic}[1]
\State \textbf{Input: } $I$, $rv$, $rv\_list$, $I\_list$, $i$
\State $I\_list[i] \leftarrow I$
\State $rv\_list[i] \leftarrow rv$
\State Return
\end{algorithmic}
\end{algorithm}





\begin{comment}
\subsection{Optimizations.}\label{Sec:Optimizations}
We use some simple static analysis techniques to put some restriction on the invariant space, which helps us to find the invariant faster.

\subsubsection{Removing Non-Iterative Precondition States}: Let $I_{iters}$ be an invariant for the CHC system: 
\begin{align*}
(\forall \vec{s}) \: P(\vec{s}) \land B(\vec{s}) &\rightarrow I(\vec{s})  \\
(\forall \vec{s},\vec{s'}) \:  I(\vec{s}) \land B(\vec{s}) \land T(\vec{s},\vec{s'}) &\rightarrow I(\vec{s'}) \\
(\forall \vec{s}) \: I(\vec{s})  &\rightarrow Q(\vec{s})  
\end{align*}
It is then trivial to see that an invariant for the standard CHC system is $(P \land \neg B) \land  I_{iters}$. This optimization reduces the search space size as the conjunctive and disjunctive size of $I_{iters}$ is lesser than or equalto the conjunctive and disjunctive size of an invariant of the standard CHC system.


\subsubsection{Affine Spaces}
A major source of poor performance is the presence of affine spaces in the program i.e. if every $s \in T^*(+_g)$ is contained in some affine space of dimension $n_0 \ge 1$. In such a case, our unoptimzed algorithm would perform a search on invariant space with size exponentially proportional to $n$, whereas an optimized search would use static techniques to find the affine space and then perform the search on invariant space with size exponentially proportional to $n - n_0 < n$, which makes a great difference. We use a modified version of Houdini's algorithm (not complete) to find affine spaces containing all eventually positive program states. We collect all coefficient-constant pairs $(\vec{w}, b)$ from $P$, $Q$ and $B$. For each coefficient-constant pair $(\vec{w}, b)$ with $\gcd \vec{w} = \vec{w}$, we first check if $(\forall \vec{x}) P(\vec{x}) \rightarrow (\vec{w}^T \vec{x} = b)$ holds, and remove those pairs for which it doesn't hold. We then check all filter out those pairs which aren't inductive i.e. which don't satisfy $(\forall \vec{x} \: \forall \vec{y}) (\vec{w}^T \vec{x} = b) \land T(x,y) \rightarrow (\vec{w}^T \vec{y} = b) $. If the set of all remaining pairs is $\mathcal{A}$, then the final affine space we report is $\bigwedge_{(\vec{w}, b) \in \mathcal{A}} (\vec{w}^T \vec{x} = b)$. The pseudocode is given below:

\begin{algorithm}[H]
\caption{Finding Affine Spaces: Modified Houdini's Algorithm.}
\begin{algorithmic}[1]
\State \textbf{Input: } $P$, $B$, $T$, $Q$
\State $\mathcal{A} \leftarrow$ GET\_COEFFICIENT\_CONSTANT_PAIRS($P$, $B$, $Q$)
\State $\mathcal{A} \leftarrow$  IMPLIES\_PRECONDITION($\mathcal{A}$, $P$)
\State $\mathcal{A} \leftarrow$  IS\_INDUCTIVE($\mathcal{A}$, $T$)
\State Return $\bigwedge_{(\vec{w}, b) \in \mathcal{A}} (\vec{w}^T \vec{x} = b)$.
\end{algorithmic}
\end{algorithm}
\end{comment}






==> sections/background.tex <==
\section{Preliminaries}
\label{sec:background}
%\gtan{Let's add a background section, which would address many of my comments later on about lacking definitions. I'll list the topics we need to cover below; you can think about in what order those should be introduced. }\ak{\checkmark}

\subsection{CHC Clause System.}
\label{subsec:chc}
A Constrained Horn Clause (CHC) system
(e.g., see~\cite{bjorner2015horn}) formally expresses the requirements for a loop invariant. Suppose we have a program with a single loop with precondition $P$, postcondition $Q$, loop guard $B$, and the loop body transition relation $T$, which relates a state before the execution of the loop body to a state after the execution. We can then construct the following CHC system:
\begin{align*}
(\forall \vec{s}) \: P(\vec{s}) &\rightarrow I(\vec{s}) &(C1) \\
(\forall \vec{s},\vec{s'}) \:  I(\vec{s}) \land B(\vec{s}) \land T(\vec{s},\vec{s'}) &\rightarrow I(\vec{s'}) &(C2) \\
(\forall \vec{s}) \: I(\vec{s})  &\rightarrow Q(\vec{s}) &(C3) 
\end{align*}
where $\vec{s},\vec{s'}$ are vectors denoting program states and $I$ is a loop invariant.  C1, C2 and C3 are called the fact, inductive, and query clauses, respectively. The fact clause (C1) states that a precondition state must be satisfied by the loop invariant, the inductive clause (C2) states that if the loop runs for a single iteration on any state satisfied by the invariant and the loop guard, the final state must also be satisfied by the invariant, and the query clause (C3) states that any state satisfying the invariant must also satisfy the postcondition \footnote{Note that the CHC clause $(\forall \vec{s}) \: I(\vec{s}) \land \neg B(\vec{s})  \rightarrow Q(\vec{s})$ is equivalent to the CHC clause $(\forall \vec{s}) \: I(\vec{s})  \rightarrow Q'(\vec{s})$ if $(\forall \vec{s}) \: Q'(\vec{s}) \leftrightarrow Q(\vec{s}) \lor B(\vec{s})$. Hence we do not have the negation of the loop guard in CHC clause $(C3)$.}.  
\stsays{why no not B in C3? it needs some explanations.} \ak{Is design choice, this choice of CHC system is able to represent some specific constructs, not possible if we use B in C3; mentioned in appendix.} \gtan{This needs to be explained in the main text or in a footnote. Honestly I still don't understand why after reading your explanation.}
The antecedent and consequent of the clauses are called body and head of the clause, respectively. \ak{Gave a footnote; I think it might explain why it is a design choice.}
%\saeid{$\vec{s}$ and $\vec{s'}$?}

\newcommand{\dstate}{\mathcal{D}_{\textit{state}}}

It is well known that finding loop invariants for the above CHC system is undecidable~\cite{blass2001inadequacy}. Practically, however, we are often interested in a finite state space, which we shall denote by $\mathcal{D}_{\textit{state}}$. {For example, if the program has $n$ signed integer variables then $\mathcal{D}_{\textit{state}} = \mathbb{Z}^n \cap \footnotesize{[- \text{INT}\_\text{MAX} - 1, \text{INT}\_\text{MAX}]}^n$, where $\footnotesize{\text{INT}\_\text{MAX}}$ is the largest integer that the system can store.}. This leads to the following bounded CHC clause system:
\begin{alignat*}{2}
(\forall \vec{s} \in \dstate) &\: P(\vec{s}) &&\rightarrow I(\vec{s})  \\
(\forall \vec{s},\vec{s'} \in \dstate) &\:  I(\vec{s}) \land B(\vec{s}) \land T(\vec{s},\vec{s'}) &&\rightarrow I(\vec{s'})  \\
(\forall \vec{s} \in \dstate) &\: I(\vec{s})  &&\rightarrow Q(\vec{s}) 
\end{alignat*}
As the invariant space for the above bounded CHC clause system is $\mathcal{P}(\dstate)$ and hence finite, finding a loop invariant for the above system is decidable. However, a naive brute force search takes $O(2^{|\dstate|})$ time, which is well beyond the limits of modern computers even for modest sized $\dstate$.

%\gtan{Let's move the rest of this subsection to the new section on problem statement and assumptions before Sec 3, as they are about limitations of our system instead of background.} \ak{\checkmark}


\subsection{Ground Positive, Ground Negative and Implication Pair States.}
We define the \emph{ground positive states} $+_g$, \emph{ground negative states} $-_g$, and \emph{ground implication pair states} $\rightarrow_g$ (called ICE pairs in \cite{garg2014ice, garg2016learning}):
\begin{align*}
    +_g &:= \{ \vec{s} \in \mathcal{D}_{\text{state}}^{n} \: : \: \vec{s} \in P \} \\
    -_g &:= \{ \vec{s} \in \mathcal{D}_{\text{state}}^{n} \: : \: \vec{s} \not\in Q \} \\
    \rightarrow_g &:= \{ (\vec{s}, \vec{s'}) \in \mathcal{D}_{\text{state}}^{2n} \: : \: \vec{s} \in B \land T(\vec{s}, \vec{s'}) \}
\end{align*}
Intuitively, a ground positive state is a state at the entry of the loop for which the precondition $P$ holds. A ground negative state is a state at the exit of the loop for which the postcondition $Q$ does \emph{not} hold. A ground implication pair state $(\vec{s}, \vec{s'})$ means that if the loop starts with state $\vec{s}$, then after one iteration the state of the program is $\vec{s'}$. From a different angle, if $\vec{s}$ is a state that is reachable from a state in $+_g$, then $\vec{s'}$ must also be a reachable state; on the other hand, if $\vec{s}$ is not reachable, there is no obligation that $\vec{s'}$ must be reachable.

\subsection{$\epsilon$-Nets.}
Our method for finding loop invariants is based on sampling using randomized $\epsilon$-nets w.r.t ellipsoids. It is defined and constructed using concepts of range spaces and Vapnik Chervonenkis (VC) dimension of range spaces. Intuitively, an $\epsilon$-net for a set $S$, w.r.t some geometrical shape such as ellipsoids, is a collection of points such that any `sufficiently' large ellipsoidal subset of $S$ must contain some point of the $\epsilon$-net. Hence if the data points we sample form an epsilon-net w.r.t ellipsoids of the set we sample from, then intuitively all counterexamples to our guessed invariant must be contained in very small ellipsoids, and if we keep tightening the maximum size of these ellipsoids with consecutive iterations, we get a convergence guarantee for our algorithm. We next define range spaces, VC dimension, and $\epsilon$-nets w.r.t any set of ranges $\mathcal{R}$, and refer to a theorem to produce an $\epsilon$ net w.r.t any set of $\mathcal{R}$ by random sampling. 

\begin{definition}
    A pair $\Sigma = (X,\mathcal{R})$, where $X$ is a non-empty set and $\mathcal{R}$ is a collection of subsets of $X$, is called a range space. Members of $\mathcal{R}$ are called ranges. $\Sigma$ is finite if $X$ is finite. 
\end{definition}

\begin{definition}
    Let $(X,\mathcal{R})$ be a range space. A finite set $A \subseteq X$ is said to be shattered by $\mathcal{R}$ if $\{ A \cap r \: | \: r \in \mathcal{R}\} = 2^{A}$. Then the Vapnik Chervonenkis (VC) dimension of $(X,\mathcal{R})$ is defined as the size of the largest\footnote{'largest' by cardinality.} subset of $X$ which is shattered by $\mathcal{R}$. \gtan{Does the "largest" here mean the largest in terms of cardinality or in terms of the subset relation? If the latter, does the largest always exist? Modify the definition to clarify this.} \ak{largest in terms of cardinality; modified}
\end{definition}

\gtan{Maybe we should give a concrete example of a range space and shattering here, using ellipsoids for $R$.}
\ak{Two interpretations of your statement: (i) Example showing largest subet of a set being shattered by ellipsoids - is extremely hard to construct; the construction and proof is the content of some other paper (and even that doesn't show exact bounds, just gives upper bounds) or (ii) Any non-largest subset of a set being shattered by ellipsoids - easy, but I wonder if this would be useful?}

 We next define $\epsilon$ nets for a range space.

\begin{definition}
    Given a finite range space $(X,\mathcal{R})$ and a parameter $0 < \epsilon < 1$, a set $N \subseteq X$ is called an $\epsilon$-net for $X$ w.r.t $\mathcal{R}$ if for every range $R \in \mathcal{R}$ s.t. $|R| \ge \epsilon |X|$, we must have $N \cap R \neq \varnothing$. \gtan{Should that be $R \in \mathcal{R}$? If $R$ is a set of sets, then we need to make clear the meaning of $|R|$ and $N \cap R$.} \ak{Yes $R \in \mathcal{R}$, changed. }
\end{definition}

Intuitively, an $\epsilon$-net $N$ for $X$ w.r.t $\mathcal{R}$ is an approximation to $X$ such that any $r \in \mathcal{R}$ must intersect $N$ or has a small (less than $\epsilon$ percentage) intersection with $X$. \gtan{Expand "s.t." to "such that", which is more appropriate in formal writing.} \ak{\checkmark}
The following theorem gives a randomized construction of an $\epsilon$ net for any finite range space of bounded VC dimension:

\begin{theorem} \cite{haussler1986epsilon}
    If $(X, \mathcal{R})$ is a finite range space of VC dimension $vc$, $\epsilon > 0$ and $m \ge \frac{8}{\epsilon}$, then a set $N \subseteq X$ obtained from $m$ uniform random independent draws from $X$ is an $\epsilon$-net for $X$ w.r.t $\mathcal{R}$ with probability strictly greater than $1 - 2 \phi_{vc}(2m)2^{-\frac{\epsilon m}{2}}$ where \
    
\begin{align*}
    \phi_d(n) &:= \begin{cases}
        \sum_{i = 0}^d \binom{n}{i}, & \mbox{if}\ d \le n \\
        2^n, &\mbox{if}\ d > n
    \end{cases}
\end{align*}
\end{theorem}
\gtan{So the above holds for arbitrary $R$? Just wanted to confirm.} \ak{Yes.}

The above theorem says that any randomly sampled subset of $X$ of `sufficient size' forms an $\epsilon$-net for $X$ w.r.t any range space with some success probability. Thus our ability to produce $\epsilon$-nets for sets of interest is dependent on whether we can randomly sample from them. We can randomly sample from a bounded polytope by using rejection sampling (described in Appendix \ref{App: Rejection Sampling}): We repeatedly uniformly sample from the axis-aligned orthotope containing the polytope until we get a sample which lies within the polytope itself. However when sampling from affine spaces, although rejection sampling still works, it is inefficient and we use an alternate technique (described in Appendix \ref{App: Sampling from Affine Spaces.}) based on sampling from the solution space of the corresponding linear diophantine equation as described in ~\cite{gilbert1990linear}.

\saeid{maybe give an intuitive how do you reject samples?}  \gtan{I think we should describe this briefly and convey the intuition.} \ak{\checkmark}

\section{Problem Statement and Assumptions.}
Our overall goal is to find an invariant that satisfies the CHC clause system stated in Section~\ref{subsec:chc}. However, we place certain restriction on the admissible formulas for precondition $P$, loop guard $B$, postcondition $Q$, transition relation $T$, and also loop invariant $I$. We now state the assumptions on the CHC clause system we wish to solve. We will discuss how these assumptions could be lifted in Section~\ref{Sec:Conclusions and Future Works.}. \gtan{I added the previous sentence; it's important to have a future work section discussing how fundamental these assumptions are and possible ways of lifting them.} \ak{I have added the reference link and written a brief section on Conclusions and Future Work.}

\begin{enumerate}
    \item We consider only programs with single loops. Programs with multiple loops require a loop invariant for each loop, which may not be reducible to the CHC clauses depending on the nesting depth of these multiple loops.
    \gtan{Do we allow programs with multiple non-nested loops? It so, maybe we should say that what we disallow is nested loops. } \ak{No, we don't allow multiple non-nested loops. Those programs more complex because: Suppose the program is L1L2 where L1 is a loop and L2 is a loop. Usually we will be given the precondition for L1 and the postcondition for L2, we will NOT be given the postcondition for L1 (which is also the precondition for L2) - so our approach doesn't solve this - we need the postcondition for negative points and we need the precondition for positive points.}

    \item We consider programs with only integer variables.
    
    \item We only consider loop programs where the propositions $P$, $B$ and $Q$ are formulas from the linear integer arithmetic (LIA) theory.
    
    \item We only consider those loop programs where $T$ is a piece-wise linear integer relation over $B$, which will be defined soon.

        \item We only consider those loop programs that admit a small sized linear invariant, i.e., an invariant which can be written as a formula from the  LIA theory with size much lesser than the size of the state space\footnote{Note that this assumption on the size of linear invariant is important, as any non-linear invariant on a finite integral state space can be written as a formula fromthe  LIA theory, albeit by using $n$ atomic predicates for each lattice point satisfying the invariant, if $n$ is the number of variables of the program.}. Such a linear invariant can always be written as a disjunctive normal formula (DNF) of atomic predicates from LIA theory, where each conjunctive clause has atmost $c$ atomic predicates, and there are atmost $d$ conjunctive clauses in disjunction with each other. \gtan{Not sure about why the small-sized part is an assumption. As far as I can see, given some c and d, we aim to find an invariant; bigger c and d just makes the algorithm run slower.} \ak{The point I am trying to make here is: Suppose the ground truth invariant is $(x \mod 3 = 1) \land (x \ge 0)$ (a non-linear invariant). As our state space is finite and integral, an alternate form of this invariant is $(x = 1) \lor (x = 4) \lor (x = 7) \lor (x = 10) \lor .. \lor (x = 10^6 - 3) \lor (x = 10^6)$ - and this form of the above invariant is a linear invariant as a DNF with $c = 2$ and $d = 10^6$ - I don't want to try to find these types of linear invariants by my method }
\end{enumerate}

We next introduce the notion of \emph{piece-wise linear integer relations} over a set. Before defining it formally, we first present some motivation. If our loop body is just a sequence of assignments whose right-hand side expressions are from the LIA theory, as in Fig \ref{Fig:LB1}, the transition relation $T$ can be written as a simple linear transformation such as $T(x,y,xp,yp) = (xp = 2x + y) \land (yp = y + 4)$. However, the presence of deterministic guard conditionals in the loop body requires that the transition relation be more general. In particular the transition relation can be a piece-wise linear function: given $B$ that partitions the state space into disjoint sets, it is a linear function on each partition set. 
For example for the loop body in Fig \ref{Fig:LB2}, our transition relation $T$ can be written as $T(x,y,xp,yp) = ((x > 5) \land (xp = 2x + y) \land (yp = y + 4)) \lor ((x \le 5) \land (xp = x + 1) \land (yp = y - 1))$. \gtan{There should be a $\lor$ somewhere in the previous formula.} \ak{\checkmark}
Now, if the loop guard has (only) nondeterministic guard conditionals, then our transition relation is the finite union of linear functions over $B$. For example in Fig \ref{Fig:LB3}, the transition relation $T$ can be written as $T(x,y,xp,yp) = ((xp = 2x + y) \land (yp = y + 4)) \lor ((xp = x + 1) \land (yp = y - 1))$. Now if our loop body consists of a mix of deterministic guard conditionals and nondeterministic guard conditionals, then the transition relation is a piece-wise linear integer relation over $B$, which is formally defined below:

\begin{definition} 
\label{Def: linear relation}
The LIA formula $T$ defines a piece-wise linear integer relation over $B$ if there exists a finite partition $\{ B_i \}$ of $B$ s.t. $B_i$ are LIA formulas for all $i$,
and $T$ when restricted on $B_i$, defined as $T_{| B_i} := \{ (x,y) \: | \: T(x,y) \land x \in B_i \}$, is a linear integer relation.
Specifically, $T_{| B_i}$ is a linear integer relation over $B_i$ if there exists a finite set of functions on $B_i$, denoted $f_{ij} : B_i \rightarrow \mathbb{R}^n$ forall $j$, where forall $j$, $f_{ij}$ is a linear function with integer coefficients only and $(\forall \vec{s} \: \forall \vec{s'}) \: T_{| B_i}(\vec{s}, \vec{s'}) \leftrightarrow \bigvee_j (f_{ij}(\vec{s}) = \vec{s'})$.

    \gtan{Don't really understand this last sentence; can you rewrite?} \ak{Rewritten, I don't know if it's clear enough though.}
\end{definition}


     
\begin{figure}
\begin{minted}{c}
    while (x + y <= 14) {
        x = 2x + y;
        y = y + 4;
    }
\end{minted}
    \caption{Loop body with terms from the LIA theory.}
    \label{Fig:LB1}
\end{figure}

\begin{figure}[H]
\begin{minipage}{.5\textwidth}
\begin{minted}{c}
    while (x + y <= 14) {
        if (x > 5) {
            x = 2x + y;
            y = y + 4;
        }
        else {
            x = x + 1;
            y = y - 1;
        }
    }
\end{minted}
    \caption{Loop body with deterministic-guard conditionals.}
    \label{Fig:LB2}
\end{minipage}%
\begin{minipage}{.5\textwidth}
\begin{minted}{c}
    while (x + y <= 14) {
        if (rand_bool()) {
            x = 2x + y;
            y = y + 4;
        }
        else {
            x = x + 1;
            y = y - 1;
        }
    }
\end{minted}
    \caption{Loop body with nondeterministic-guard conditionals.}
    \label{Fig:LB3}
\end{minipage}%
\end{figure}

A CHC clause system which satisfies (1) - (4) is called a standard linear CHC clause system for a single loop. A standard linear CHC clause system for a single loop allows us to encode a large class of single loop programs, which use constructs like random initialization of variables, nondeterministic loop guards, conditionals with deterministic and nondeterministic guards,  \texttt{break}/\texttt{continue}
statements, and  \texttt{goto} statements. We demonstrate the encoding of such constructs via examples in Appendix~\ref{App: Representing Practical Programs in the Standard CHC Clause system}.

\begin{comment}
\begin{itemize}
    \item The CHC system from a prgram with a loop, pre-, and post-condition.
    \item Positive, negative, and implicattion sets
    \item epsilon-nets? Not sure if this should go here, but in the overview we mention it.
\end{itemize}
\end{comment}

==> sections/intro.tex <==
\section{Introduction}
\label{sec:intro}
% \gtan{Maybe it helps to have a catchy name for the system?} \jz{What about \toolname? D for Data-drive and $LIA^2$ for LIA Loop Inv Auto.}

The formal verification of software code for safety and security requirements such as memory safety, termination guarantees, and information leaks is crucial to safeguarding critical infrastructures against intentional and unintentional risks.
Since existing unverified software is too large to be verified manually, researchers have turned to building tools that automate the verification of safety and security properties. One prevalent method in automated formal
verification is Hoare Logic~\cite{hoare1969axiomatic}: it reduces the problem of verifying the whole program w.r.t a given property to verifying each program statement separately with a given pre- and post-condition. 

Loops, however, pose significant challenges to Hoare-Logic based verification since the verification has to supply  a special type of proposition called \emph{loop invariants}. 
Intuitively, a loop invariant is a proposition that is \texttt{true} at the beginning of the loop and remains \texttt{true} for each iteration of the loop body. 


\begin{comment}
\gtan{I am moving the following CHC discussion to the background.}

A Constrained Horn Clause (CHC) system\footnote{This CHC clause corresponds to a single loop program. Programs with multiple loops require a loop invariant for each loop, which may not be reducible to the above CHC clause depending on the nesting depth of these multiple loops. For this paper, we  consider only programs with single loops and from now on shall refer to single loop programs as loop programs. \gtan{This is an important limitation of the tool; we should elevate this to the main text, moving it to a place where we collect all assumptions.}
} (e.g., see~\cite{bjorner2015horn}) can formally express the requirements for a loop invariant. 

For a program with a single loop with precondition $P$, postcondition $Q$, loop guard $B$, and the loop body transition relation $T$ (which relates a state before the body to a relate after the body execution), we have the following CHC system:
\begin{alignat*}{2}
(\forall \vec{s}) &\: P(\vec{s}) &&\rightarrow I(\vec{s})  \\
(\forall \vec{s},\vec{s'}) &\:  I(\vec{s}) \land B(\vec{s}) \land T(\vec{s},\vec{s'}) &&\rightarrow I(\vec{s'})  \\
(\forall \vec{s}) &\: I(\vec{s}) \land \neg B(\vec{s})  &&\rightarrow Q(\vec{s}) 
\end{alignat*}
where $\vec{s},\vec{s'}$ are vectors denoting program states and $I$ is a loop invariant. 
%\gtan{We should consider whether it's possible to rewrite the intro without giving listing the detailed clauses in a CHC system; if you keep the above clauses in the intro, we need to explain each clause briefly.}

It is well known that finding loop invariants for the above CHC system is undecidable~\cite{blass2001inadequacy}. Practically, however, we are interested in a finite state space, which we shall denote by $\mathcal{D}_{\textit{state}}$\footnote{For example if the program has $n$ integer variables then $\mathcal{D}_{\textit{state}} = \mathbb{Z}^n \cap \footnotesize{[- \text{INT}\_\text{MAX} - 1, \text{INT}\_\text{MAX}]}^n$ where $\footnotesize{\text{INT}\_\text{MAX}}$ is the largest integer the system can store.}. This leads to the following bounded CHC clause system:
\begin{alignat*}{2}
(\forall \vec{s} \in \mathcal{D}_{\textit{state}}) &\: P(\vec{s}) &&\rightarrow I(\vec{s})  \\
(\forall \vec{s},\vec{s'} \in \mathcal{D}_{\textit{state}}) &\:  I(\vec{s}) \land B(\vec{s}) \land T(\vec{s},\vec{s'}) &&\rightarrow I(\vec{s'})  \\
(\forall \vec{s} \in \mathcal{D}_{\textit{state}}) &\: I(\vec{s}) \land \neg B(\vec{s})  &&\rightarrow Q(\vec{s}) 
\end{alignat*}
As the invariant space for the above bounded CHC clause system is finite, finding a loop invariant for the above system is decidable. \gtan{This depends on how you define the invariant space; it won't be finite if the coefficients can be real numbers.} However, a naive brute force search takes $O(2^{|\mathcal{D}_{\textit{state}}|})$ time, which is well beyond the limits of modern computers.\gtan{The previous statement depends on how big the domain is.}
\end{comment}

It is well known that finding loop invariants is undecidable~\cite{blass2001inadequacy}. However, previous practical approaches have had
success by limiting the invariant search space. 
Previous techniques for finding loop invariants can be broadly classified into static or data-driven, based on whether they use runtime program data or not.  Static techniques usually come with completeness guarantees for finding a loop invariant, albeit only for a restricted subclass of loop programs. \ak{May have to remove these sentences all together}  Data-driven techniques are known to  perform well experimentally on a broader class of programs when compared to their static counterparts, but they
come with no completeness guarantees in finding loop invariants, even for linear loops (i.e., loops where all assignments and guards are linear expressions of program variables). \saeid{we need citations for these works. do we have a list?} \ak{Added some references, I will read more papers on Invariant Automation, to get a list.}

We present the first data-driven technique with probabilistic guarantees for finding linear loop invariants of programs with integer variables.  We use a guess-and-check algorithm (~\cite{garg2016learning, garg2014ice, krishna2015learning, nguyen2017counterexample, zhu2018data}) to compute the loop invariant. At the high level, a guess-and-check algorithm iteratively produces guess invariants to a CHC clause, and uses a SMT solver to verify these guesses. Typically this has a reinforcement component to it: if the SMT solver rejects a guess, it also gives a set of counterexamples which the guess algorithm can use to `refine' the `quality' of their guesses. 

In the guess-phase of our algorithm (which we refer to as the Simulated Annealing Loop), we sample a dataset of positive, negative and implication pair (~\cite{garg2014ice}) points from the CHC clause system. We use the concept of $\epsilon$-nets (\cite{haussler1986epsilon}) here: our positive, negative and implication pair points form an $\epsilon$-net of the respective sampling regions. This allows us to give termination guarantees on the check-phase of our algorithm. We design a novel distance-based cost function, which is zero iff a candidate guess invariant satisfies the approximate CHC clause system i.e. the CHC clause system when quantified only over our sampled data-set instead of the full state space. Intuitively, this cost function measures how 'far' our current guess invariant is from satisfying the approximate CHC clause system. We use a multi-threaded simulated annealing search (\cite{mitra1986convergence}) to find a guess invariant satisfying the approximate CHC clause system. Our simulated annealing approach is geometrically motivated: we use $n$-dimensional translations and $n$-dimensional rotations of the boundary hyperplanes as our SA transitions.

In the check-phase of our algorithm (which we refer to as the Datapoint Sampling Loop), we verify our approximate invariant on the CHC clause system using a SMT solver like Z3 (~\cite{de2008z3}). If it is not a correct invariant, we add the counterexamples generated by the SMT solver to our datapoints. Additionally, we also 'tighten' the $\epsilon$-net periodically. Our guess-and-check approach demonstrates that guess-and-check algorithms can come with completeness guarantees on finding invariants for a sufficiently large class of loop programs. 


\saeid{we need to give some insights about the novelty and significant of findings.} \gtan{We need to write a bit more about the insights. Start by describing the guess and check approach (can we say we are the first to attempt it?),
and then briefly describes our epsilon-net based sampling approach, which ensures termination. Maybe also describe our novel combination of counter examples with sampling. In general, this is where we sell the work; so we need to write several paragraphs to highlight contributions.
}
\ak{\checkmark. Added 2 paragraphs above.}

Although loop programs with linear loop invariants theoretically form a small subclass of loop invariants, in practice, they form the bulk of the required loop invariants for loop programs. We report good experimental results on the benchmarks tested. Additionally, our approach serves as a case study for when simulated annealing outperforms gradient descent.


We organize our paper as follows. Section \autoref{Sec:Overview} describes the overview of our algorithm via an example. Section \autoref{Sec:Standard CHC clause and Classification of Datapoints} formally defines the CHC clause system, the state space, and $d$-$c$ LIA invariants. Section \autoref{Sec:Algorithm} describes our complete algorithm, in which subsection \autoref{SubSec:CEGIS Loop} defines the Datapoint Sampling loop and subsection \autoref{SubSec:SA Loop} describes the simulated annealing loop. Section \autoref{Sec:Convergence Guarantees} describes our convergence results. Section \autoref{Sec:Tool and Experiments} gives the outline of our tool and our results, and compares our methodology with other existing tools. Section \autoref{Sec:Conclusions and Future Works.} describes conclusions and future work.



==> sections/overview.tex <==
\section{Overview}
\label{Sec:Overview}

\begin{figure}[!tbh]
\begin{minted}{c}
int main(void) {
    int x = 1;
    int y = 1;
    while (rand_bool()) {
        x = x + y;
        y = x;
    }
    assert (y >= 1);
    return 0;
}
\end{minted}
    \caption{An example \texttt{C} program that requires $y \geq 1 $ after the loop.}
    \label{eg1}
\end{figure}

We describe a brief overview of our algorithm via an example. Consider the example \texttt{C} code in Fig \ref{eg1} .
For the above example, a loop invariant for the while loop is a predicate over the integer variables $x$ and $y$ denoted by $I(x,y)$, which satisfies the following bounded CHC clause system:
\begin{alignat*}{2}
    (\forall x,y \in \mathcal{D}_{\text{int}}) &\: (x = 1) \land (y = 1) &&\rightarrow I(x,y) \\
    (\forall x,y, x', y'\in \mathcal{D}_{\text{int}}) &\: I ( x,y ) \land (x' = x + y) \land (y' = x') &&\rightarrow I(x', y') \\
    (\forall x,y \in \mathcal{D}_{\text{int}}) &\:I(x,y) &&\rightarrow y \ge 1
\end{alignat*}
where $\mathcal{D}_{\text{int}} := \mathbb{Z} \cap \footnotesize{[- \text{INT}\_\text{MAX} - 1, \text{INT}\_\text{MAX}]}$.
\gtan{We should move the following few sentences to the beginning of the problem statement section. This is the goal of our system and part of the problem statement.} \ak{This is there, and in more detail. It is part 5 of that assumptions list over there.}
We are interested in finding loop invariants that can be written as the disjunction of $d$ clauses, where each clause is the conjunction of atmost $c$ closed hyperplanes for some natural numbers $c$ and $d$ (which are provided by user); such invariants can be viewed geometrically as the lattice points contained in a finite union of $d$ convex compact polytopes with atmost $c$ faces. For the above example, we set $c = 2$ and $d = 1$.

Our algorithm comprises two nested loops as depicted in Fig \ref{fig:DSSA Connection}. The outer loop, called the DS (Datapoint Sampling) loop approximates the bounded CHC system above with a version with smaller domains of quantification; in detail, at iteration $k+1$ it finds $+_k$, $-_k$ and $\rightarrow_k$ sets s.t. the approximate CHC system is:
%\gtan{In the background section, we discussed only ground positive states, not general positive states. Maybe in the background, we should also define what generally positive, negative, implication pair states mean.} \saeid{maybe let's just explain the three sets instead of following equations.} \ak{@GT, @Saeid: This information is defined in detail in the next section, which bits should I move earlier?} 

\begin{alignat*}{2}
    (\forall (x,y) \in +_k) &\: (x = 1) \land (y = 1) &&\rightarrow I(x,y) \\
    (\forall ((x,y) , (x', y')) \in \: \rightarrow_k) &\: I ( x,y ) \land (x' = x + y) \land (y' = x') &&\rightarrow I(x', y') \\
    (\forall (x,y) \in -_k) &\:I(x,y) &&\rightarrow y \ge 1
\end{alignat*}

\begin{figure}
    \centering
    \includegraphics[scale = 0.18]{sections/DSSAConnection.png}
    \caption{Diagram showing input-output behavior of DS and SA Loops. \gtan{This figure is quite unclear. Let's use a CFG-like structure shown in Fig~\ref{fig:cfg}, which shows the nested structure. Free free to add more boxes, but you shouldadd the right description into each box and label edges with the right conditions. Another possibility is to use some pseudo code.} }
    \label{fig:DSSA Connection}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale = 0.1]{Figures/cfg.png}
    \caption{Diagram showing input-output behavior of DS and SA Loops.}
    \label{fig:cfg}
\end{figure}

 The inner loop, called the Simulated Annealing (SA) loop, tries to find a correct invariant of the above  approximate CHC system---such an invariant is called an approximate invariant. \gtan{In latex, single dash "-" is different from three dashes "---"; grammatically, you should use three dashes above or just a semicolon. I noticed many places where this happend.}
 \ak{I will change this wherever I observe this; but since we have divided each section into separate latex files, Overleaf's regex matching only works for individual file, doing for all files separately is too much work.} \gtan{Maybe combine all files into one; there's really no need to have separate files IMO.}
 %For each iteration $k+1$ of the DS loop, let $(+_k, -_k, \rightarrow_k)$ denote the domains of quantification we have at the start of iteration $k+1$ of the DS loop.

 %\gtan{We need to explain what epsilon nets are; not in details, but an intuition should be fine in the overview. Say something like it's an way of sampling the domains.}
 
 We take $+_0, -_0,$ and $ \rightarrow_0$ to be $\epsilon$-nets of $(x = 1) \land (y = 1)$, $\neg (y \ge 1)$, and $\{  ((x,y) , (x + y,x + y)) \: | \: \neg((x = 1) \land (y = 1)) \land  (y \ge 1) \}$ w.r.t ellipsoids respectively.
 Intuitively, an $\epsilon$-net of a set $S$ w.r.t ellipsoids is some subset of $S$ denoted $X$ s.t. any ellipsoidal shaped subset of $S$ of `sufficient' size meets $X$---for our application, the ellipsoidal shaped subsets are counterexamples to an approximate invariant and casting an $\epsilon$-net ensures that we can bound the number of such counterexamples possible.
  This, combined with decreasing $\epsilon$ ensures convergence of the DS loop.
{By an $\epsilon$ net of $\{  ((x,y) , (x + y,x + y)) \: | \: \neg((x = 1) \land (y = 1)) \land  (y \ge 1) \}$  w.r.t ellipsoids, we mean the set $\{  ((x,y) , (x + y,x + y)) \: | \: (x,y) \in H \}$ where $H$ is an $\epsilon$-net of $\neg((x = 1) \land (y = 1)) \land  (y \ge 1)$ w.r.t ellipsoids.}. 

 For subsequent iterations of the DS loop, we update our domains of quantification using an SMT solver (e.g., Z3) as a teacher in a feedback loop\footnote{This is possible as Linear Integer Arithmetic (LIA) satisfiability is decidable.}: we check if the approximate invariant satisfies the original (unapproximated) bounded CHC system. If yes, we just find our loop invariant. Otherwise, we ask the SMT solver for a small set of counterexamples $(+^\times_k, -^\times_k, \rightarrow^\times_k)$ which we append to our current domain of quantification: i.e., $(+_{k+1}, -_{k+1}, \rightarrow_{k+1}) = (+_k \sqcup +^\times_k, -_k \sqcup -^\times_k, \rightarrow_k \sqcup \rightarrow^\times_k)$ and go to the next DS loop iteration. \gtan{Is there a reason we are not using the set union symbol ($\cup$) in the above?} \ak{We just using $\sqcup$ which means disjoint union - which is effectively the union, but also conveys the fact that the individual sets on either side of $\sqcup$ are disjoint.}
 Additionally, at periodic intervals, we substitute our $\epsilon$-net with a `tighter' net i.e. a $\epsilon'$-net for $0 < \epsilon' < \epsilon$. This ensures the termination of the DS Loop.


In the SA loop we search for the approximate invariant by running a simulated annealing search ~\cite{mitra1986convergence} on the candidate invariant space: a candidate invariant is the union of any $d$ polytopes, each with at most $c$ faces (for this example a candidate invariant is the intersection of two halfplanes.).
\gtan{Provide a citation for SA above. Also, why "approximate" invariant? I thought it would be a true invariant for the approximated system.} \ak{citation added. The terminology we use: (i) True invariant of just invariant is referred to the invariant which satisfies the CHC clause system, or can be called the ground truth invariant, (ii) Approximate invariant: Any invariant for the approximated system and (iii) Candidate Invariant: Literally any invariant from the search space.}
In this search, our neighbors are defined by a translation or 2-dimensional rotation of some boundary line of some halfplane of the original candidate invariant and our cost function is defined as a linear-time approximation to the set-distance metric. Additionally, we use multiple threads within the SA loop to increase the probability of finding the approximate invariant. 
% \saeid{we need to stay a bit high-level in the overview: we just need to say what is goal, what method we used to achieve the goal, and what are the concrete outputs for the C code. I like this paragraph more than the one before because of simplicity.} \saeid{let us brainstorm how to merge inner and outer loop.} \ak{\checkmark}

For the example given above, Figure \ref{Fig:stateSpacePlot} depicts a graphical description of a SA run for a single thread at 4 different time intervals for the 1st DS loop iteration. From these above plots, we can also visualize the structure of $\epsilon$-nets for the $-$ and $\rightarrow$ domain of quantification. 
\saeid{The plots are very nice, but we did not utilize (sell) them well in the current version.} \ak{I give a description of the plots in the caption, should I move this to main text?} 

% Uncomment this when you need to see it, otherwise don't else document takes too much time to compile

 \begin{comment} 
\begin{figure}
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/SA1.pdf}
  \includegraphics[width=\linewidth]{Figures/SA3.pdf}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/SA2.pdf}
  \includegraphics[width=\linewidth]{Figures/SA4.pdf}
\end{minipage}
\caption{This figure shows a SA run for a thread for the 1st DS loop iteration for Example \ref{eg1}. The blue arrows represent shows implication pairs, a red ($-$) represents a minus datapoint, and the green ($+$) shows
the single plus datapoint, located near the origin. The candidate invariant currently being considered is outlined by black and it's interior is shaded in gray. The topleft, topright, bottomleft, and bottomright show the candidate invariant changes by a single rotation or translation over one of its boundary lines (1D faces). }
\label{Fig:stateSpacePlot}
\end{figure}

\end{comment}


==> sections/related-work.tex <==
\section{Conclusions and Future Works.}
\label{Sec:Conclusions and Future Works.}
Our tool \toolname{} is the first guess-and-check algorithm which comes with theoretical guarantees on the success probability of finding the invariant. Our experimental evaluation yields good results and are comparable with state of the art tools.

\ak{This next paragraph mentions possible future directions of work - I want to mention this, but also not give away information as to how to approach these new problems.}
Our approach however does make some assumptions on the CHC clause system. (1) We firstly assume that our CHC clause system only models a program with a single loop. Programs with nested loop have an loop invariant at each depth and require a more-complicated analysis on the search space. Programs with sequential loops usually have the same structure for the CHC clause for each loop in the sequential loop program but often precondition and postcondition states are missing for the internal loops in the sequential loop program. We propose address these issues as a future derivative study of this one.
(2) We only consider programs with integer variables: We propose to extend our method to real variables as well as a future work. (3) We only consider programs where $P$, $B$ and $Q$ are LIA formulas, T is a piecewise linear relation over $B$ and our invariant search space comprises only of linear invariants. We propose to extend our approach to incorporate polynomial invariants and non-linear formulae for $P$, $B$ , $Q$ and $T$. An orthogonal extension is to allow data structures like arrays and pointers in our background theory: our resultant guess and check becomes more complicated.


In an orthogonal direction, our approach demonstrates an instance when a simulated annealing search on the search space is more useful than convention ML-based gradient descent searches.


